Token-Level LLM Collaboration via FusionRoute

Large language models (LLMs) exhibit strengths across diverse domains. However, achieving strong performance across these domains with a single general-purpose model typically requires scaling to sizes that are prohibitively expensive to train and deploy. On the other hand, while smaller domain-specialized models are much more efficient, they struggle to generalize beyond their training distributions. To address this dilemma, we propose FusionRoute, a robust and effective token-level multi-LLM collaboration framework in which a lightweight router simultaneously (i) selects the most suitable expert at each decoding step and (ii) contributes a complementary logit that refines or corrects the selected expert's next-token distribution via logit addition. Unlike existing token-level collaboration methods that rely solely on fixed expert outputs, we provide a theoretical analysis showing that pure expert-only routing is fundamentally limited: unless strong global coverage assumptions hold, it cannot in general realize the optimal decoding policy. By augmenting expert selection with a trainable complementary generator, FusionRoute expands the effective policy class and enables recovery of optimal value functions under mild conditions. Empirically, across both Llama-3 and Gemma-2 families and diverse benchmarks spanning mathematical reasoning, code generation, and instruction following, FusionRoute outperforms both sequence- and token-level collaboration, model merging, and direct fine-tuning, while remaining competitive with domain experts on their respective tasks.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{url}
\usepackage{subcaption}

\usepackage{colortbl}
\usepackage{xcolor}

\usepackage{graphicx}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{float}

\usepackage{booktabs}

\usepackage{enumitem}

\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newcommand{\hz}[1]{{\color{teal}Hanqing:[#1]}}
\newcommand{\AAA}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\OOmega}{\mathbb{\Omega}}

\newcommand{\rA}{\mathscr{A}}
\newcommand{\rB}{\mathscr{B}}
\newcommand{\rC}{\mathscr{C}}
\newcommand{\rD}{\mathscr{D}}
\newcommand{\rE}{\mathscr{E}}
\newcommand{\rF}{\mathscr{F}}
\newcommand{\rG}{\mathscr{G}}
\newcommand{\rH}{\mathscr{H}}
\newcommand{\rI}{\mathscr{I}}
\newcommand{\rJ}{\mathscr{J}}
\newcommand{\rK}{\mathscr{K}}
\newcommand{\rL}{\mathscr{L}}
\newcommand{\rM}{\mathscr{M}}
\newcommand{\rN}{\mathscr{N}}
\newcommand{\rO}{\mathscr{O}}
\newcommand{\rP}{\mathscr{P}}
\newcommand{\rQ}{\mathscr{Q}}
\newcommand{\rR}{\mathscr{R}}
\newcommand{\rS}{{\mathscr{S}}}
\newcommand{\rT}{{\mathscr{T}}}
\newcommand{\rU}{\mathscr{U}}
\newcommand{\rV}{\mathscr{V}}
\newcommand{\rW}{\mathscr{W}}
\newcommand{\rX}{\mathscr{X}}
\newcommand{\rY}{\mathscr{Y}}
\newcommand{\rZ}{\mathscr{Z}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tex/ablation.tex <==
\section{Ablation Study}
\subsection{Ablation on Complementary Logit Contribution}\label{subsec:ablation_complement}
% \nuoya{Do we need Collab as a baseline to show that our routing mechanism works better than Collab?}
% \paragraph{Role of complementation} 
We first examine the role of the router's complementary logit contribution in \algname.
%
In particular, we aim to isolate whether token-level expert selection alone is sufficient for effective collaboration, or whether the router's ability to directly contribute corrective logits is necessary for strong performance.
%
% We first present empirical evidence showing that the router's complementary mechanism plays a critical role in achieving strong performance, and that token-level multi-agent collaboration alone is insufficient to deliver satisfactory results.   
%
To this end, we construct a routing-only baseline that removes the complementary component: we use the router obtained after the SFT phase to select an expert at each token, and generate the next token solely from the selected expert's logits, without adding the router's logits.
%
% \begin{wrapfigure}{r}{0.45\linewidth}
%     % \vspace{-10pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ablation.png}
%     \caption{
%     GPT-4o winrate comparison: with vs. without complementation on both Llama-3 and Gemma-2 Family.
%     \zz{Debatable if we want to keep this figure since this is not an apple-to-apple comparison considering it is SFT checkpoint vs. SFT+CDPO. Maybe we can delete this win rate figure and just use it in 6.2?} \yh{I think our aim for this figure is not make an apple-to-apple comparison but to show our complementation has the incremental value?}
%     }
%     \vspace{-10pt}
%     \label{fig:winrate_ablation}
% \end{wrapfigure}
%
% For the baseline without the complement part, we use the router after the SFT phase for purely token-level routing. 
%
% We do not use the router trained after CDPO because, although CDPO improves final performance, it slightly disrupts the router’s routing behavior.  
%
% Then, for each token, we follow the router to select the candidate model and use the candidate model's logits as the final logits. 
%

\tabref{table:ablation_pms} reports the cross-domain performance of the routing-only variant compared with the full \algname framework across both the LLaMA-3 and Gemma-2 families. 
%
We see that \algname consistently outperforms \algname w/o complementary logits across nearly all benchmarks and both model families. 
%
The performance gap is particularly pronounced on coding and instruction-following tasks, where even correctly selected experts can produce locally suboptimal or misaligned tokens that require correction.
%
% \tabref{table:ablation_pms} compares \algname with and without complementary logits on both the LLaMA-3 and Gemma-2 model families. 
%
% \figref{fig:winrate_ablation} shows that \algname with router complementation outperform pure token-level routing. 
%
% This demonstrates that the router's complementary mechanism is essential for effective collaborative decoding across multiple LLMs and further supports our theoretical analysis (\secref{sec:theoretical_analysis}) about the limitations of purely token-level routing.  
These results provide direct empirical evidence support for our theoretical analysis in \secref{sec:theoretical_analysis}. 
%
Even when the router is able to identify a suitable expert at each token, relying solely on fixed expert logits is insufficient to reliably recover a near-optimal policy.
%

%
In contrast, allowing the router to contribute complementary logits effectively expands the expressive capacity of the decoding policy, enabling it to correct expert failures and achieve stronger, more robust performance across heterogeneous domains.
%
%

Moreover, we find that the routing-only variant (\algname w/o complementary logits) already  outperforms the state-of-the-arts controlled-decoding-based token-level collaboration method~\citep{chakraborty2025collab} across most benchmarks. 
%
This improvement suggests that directly training the routing component on expert data is crucial for learning accurate and stable token-level routing behaviors. 
%
In contrast, controlled-decoding approaches that rely solely  on external reward signals tend to exhibit higher 
instability, limiting their effectiveness in practice.
%
%
% We also evaluate the cross-domain performance of pure token-level routing versus \algname, as shown in \tabref{table:ablation_pms}, where \algname outperforms pure token-level routing in nearly all tasks, highlighting the importance of the complementary mechanism.
%





% \textbf{Discussion 1: Complementation is More Beneficial at Larger Scale} We find that the role of complementation becomes more obvious in the larger 8B model family. In the large-model setting, the router exhibits greater flexibility and capacity, enabling it to more effectively learn how to act as a complementary generator. In contrast, smaller models have relatively limited representational ability, making it more difficult for the router to learn strong complementary behaviors, and thus the performance gains are less substantial.

% \textbf{Discussion 2: Our Pure Token-Wise Routing is Better than the Previous Token-Level Collaboration Approach} 

%
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} 
& \textbf{GSM8K} 
& \textbf{MATH500} 
& \textbf{MBPP} 
& \textbf{HumanEval} 
& \textbf{IFEval} 
& \textbf{Avg Acc.} \\
\midrule
\multicolumn{7}{c}{\textit{Llama-3 Family}} \\
\midrule
Collab 
& 0.82 & 0.32 & \underline{0.28} & 0.54 & 0.55 & 0.502 \\
% Pure Token-Level Routing 
\algname w/o complementary logits
& \underline{0.82} & \underline{0.32} & 0.26 & \underline{0.56} & \underline{0.65} & \underline{0.522} \\
\rowcolor{blue!10}\algname 
& \textbf{0.82} & \textbf{0.33} & \textbf{0.36} & \textbf{0.63} & \textbf{0.69} & \textbf{0.566} \\
\midrule
\multicolumn{7}{c}{\textit{Gemma-2 Family}} \\
\midrule
Collab 
& 0.52 & 0.22 & \textbf{0.26} & \underline{0.35} & 0.45 & 0.360 \\
% Pure Token-Level Routing 
\algname w/o complementary logits
& 0.62 & \textbf{0.23} & 0.23 & 0.33 & \underline{0.51} & \underline{0.384} \\
\rowcolor{blue!10}\algname 
& \textbf{0.65} & \underline{0.22} & \underline{0.25} & \textbf{0.40} & \textbf{0.61} & \textbf{0.426} \\
\bottomrule
\end{tabular}
\caption{
    Cross-domain performance comparison between purely token-level routing and \algname across model families.
    %
    Best and second-best performance within each family are highlighted by \textbf{bold} and \underline{underline}, respectively.
    %
}
\label{table:ablation_pms}
\end{table*}
%


% \begin{table}[t]
% \centering
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg\\
% \midrule
% Collab & 0.82 & 0.32 & 0.28 & 0.54 & 0.55 & 0.502 \\
% Purely Token-Level Routing  & 0.82 & 0.32 & 0.26 & 0.56 & 0.65 & 0.522\\
% \algname & 0.82 & 0.33 & 0.36 & 0.63 & 0.69 & \textbf{0.566} \\
% \bottomrule
% \end{tabular}
% \caption{Llama-3 Family}
% \end{subtable}
% \\ \vspace{1em}
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg\\
% \midrule
% Collab & 0.52 & 0.22 & 0.26 & 0.35 & 0.45 & 0.360 \\
% Purely Token-Level Routing & 0.62 & 0.23 & 0.23 & 0.33 & 0.51 & 0.384 \\
% % SFT DPO Mix Training & 64.75 & 23.0 & 24.6 & 41.4 & 59.23 & 0.427 \\
% \algname & 0.65 & 0.22 & 0.25 & 0.40 & 0.61 & \textbf{0.426} \\
% \bottomrule
% \end{tabular}
% \caption{Gemma-2 Family}
% \end{subtable}
% \caption{Cross-domain performance of purely token-level routing and \algname. }\label{table:ablation pms}
% \end{table}


\subsection{Ablation on \algname Training Procedure}
% \begin{wrapfigure}{r}{0.45\linewidth}
%     \vspace{-0.7in}
%     \centering
%     \includegraphics[width=\linewidth]{figures/ablation_sft.png}
%     \caption{
%     GPT-4o winrate comparison: \algname with vs. without CDPO training on both Llama-3 and Gemma-2 Family.
%     %
%     % \zz{blue is kind of reserved to DARE as in Figure 3, maybe just a lighter orange (to indicate they are the similar method)? also make the legends, labels even bigger? also remove the fig title}
%     }
%     \vspace{-0.2in}
%     \label{fig:winrate_ablation_sft}
% \end{wrapfigure}
While the ablation in \secref{subsec:ablation_complement} demonstrates the importance of complementary logits at inference time, it does not 
examine how different stages of the \algname training procedure contribute to this behavior. 
%
In this section, we further probe the training pipeline of \algname by ablating the preference-optimization stage, with the goal of understanding the effectiveness of the proposed CDPO over SFT. 
%
To this end, we compare three variants: a base model, \algname after the SFT phase, and the full \algname framework with CDPO training.
%
We evaluate these variants using GPT-4o win rate on a held-out general dataset, which captures overall response quality beyond task-specific correctness.
%
% Combining the results in \tabref{table:main} and \figref{fig:winrate}, we observe that the CDPO phase in our \algname training does not improve cross-domain performance, but it significantly increases GPT-4o win rate on general datasets. 
%
% This suggests that the primary benefit of the DPO-based complement training is to enhance general response quality such as formatting and alignment with human preferences. 
%
% To more directly demonstrate the benefit of complementary training, we further evaluate the GPT-4o win rate of responses generated by \algname after the SFT phase, and compare it with both the directly fine-tuned model and the full \algname framework.
%


The result are shown in \figref{fig:winrate_ablation_sft}. 
%
We observe that while SFT already provides a reasonable initialization, \begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{figures/ablation_sft.png}
    \vspace{-10pt}
    \caption{
    GPT-4o winrate comparison: \algname\ with vs.\ without CDPO training on both Llama-3 and Gemma-2 families.
    }
    \label{fig:winrate_ablation_sft}
    \vspace{-10pt}
\end{wrapfigure}applying CDPO training leads to a substantial improvement in win rate. 
%
In particular, the full \algname model significantly
 outperforms its SFT-only counterpart, indicating that the complementary component learned during CDPO effectively corrects expert failures and enhances the overall response quality.
%
These findings suggest that the performance gains of \algname depend critically on the preference-optimization stage in the training procedure, which substantially improves general response quality.
% This ablation study thus provides direct evidence that DPO-based complementary training is a crucial contributor to the performance gains of \algname, rather than a byproduct of supervised fine-tuning alone.
%
%
%
% In contrast, task-specific correctness or accuracy (e.g., in mathematics or coding) is largely determined by the candidate models and the router’s token-level routing component.
%

==> tex/abstract.tex <==
% Alignment has become increasingly important for LLM to further improve a model’s capabilities. 
% \zz{
Large language models (LLMs) exhibit strengths across diverse domains.
%
However, achieving strong performance across these domains with a \textit{single} general-purpose model typically requires scaling to sizes that are prohibitively expensive to train and deploy. 
%
On the other hand, while smaller domain-specialized models are much more efficient, they struggle to generalize beyond their training distributions.
%
% }
%
% However, a single model often struggles to handle diverse downstream tasks such as mathematics, coding, and instruction following. 
%
% Therefore, effectively leveraging off-the-shelf expert models becomes essential for building a comprehensive model framework. 
%
% Token-level multi-LLM collaboration offers a natural Mixture-of-Agent (MoA) paradigm that enables different expert models to work together without requiring gradient access or additional joint training, as is typically needed in Mixture-of-Experts (MoE). 
%
% However, the exploration of how to effectively select the appropriate expert at the token level and correct or guide the expert when it fails remains limited.
%
To address this dilemma, we propose \algname, a robust and effective token-level multi-LLM collaboration framework 
% by training a router that 
in which a lightweight router
simultaneously (i) selects the 
% appropriate expert for next-token prediction, 
most suitable expert at each decoding step
and (ii) 
% provides a complementary part of the selected models' generation.
contributes a complementary logit that refines or corrects the selected expert's next-token distribution via logit addition.
%
% Theoretically, we show that our model selection strategy is significantly more effective than existing approaches, and relying solely on expert models for token-level collaboration is fundamentally limited in achieving the optimal value function. 
%
% In contrast, our framework with a base-model prior can reach the optimal value function.
%
% \zz{
Unlike existing token-level collaboration methods that rely solely on fixed expert outputs, we provide a theoretical analysis showing that pure expert-only routing is fundamentally limited: unless strong global coverage assumptions hold, it cannot in general realize the optimal decoding policy. 
%
By augmenting expert selection with a trainable complementary generator, \algname expands the effective policy class and enables recovery of optimal value functions under mild conditions.
%
% }
Empirically, 
% comprehensive evaluations across multiple domains and general datasets demonstrate that our approach achieves state-of-the-art cross-domain performance and the highest GPT win rate on general datasets.
% \zz{
across both Llama-3 and Gemma-2 families and diverse benchmarks spanning mathematical reasoning, code generation, and instruction following, \algname outperforms both sequence- and token-level collaboration, model merging, and direct fine-tuning, while remaining competitive with domain experts on their respective tasks.
%
% }


==> tex/conclusion.tex <==
\section{Conclusion}
In this paper, we present \algname, a framework that enables multiple candidate models to collaboratively generate higher-quality responses than any individual model. 
%
\algname works well automatically across diverse scenarios because of a routing mechanism, and provides robustness by letting the router provide complementary logits to refine the overall response quality. 
%
In addition, \algname is computationally efficient, as it avoids requiring each model to generate candidate tokens or full responses for selection. 
%
Theoretically, we characterize the limitations of purely token-level collaboration and demonstrate the benefits of incorporating complementary logits. 
%
Extensive experiments on both domain-specific and general datasets verify the effectiveness of our framework.
%

==> tex/experiments.tex <==
\section{Experiments}
In this section, we first describe the experimental setup in \secref{sec:exp setup}.
%
We then present cross-domain performance and win rates on general benchmarks in \secref{sec:exp_crossdomain}. 
%
% Together, these evaluations demonstrate that our \algname enables effective collaboration among multiple models by (a) selecting the most domain-appropriate models for accurate specialized responses and (b) delivering consistently high-quality outputs on general datasets.
Together, these results show that \algname enables effective multi-model collaboration by selecting domain-appropriate experts while maintaining strong performance on general tasks.
%


\subsection{Experimental Setup}\label{sec:exp setup}
\paragraph{Baselines.}
We compare \algname against a broad set of baselines, including sequence-level collaboration, token-level collaboration, model merging, and single-model fine-tuning.
% We include several popular types of approaches for multi-LLM collaboration as our baselines. 
%
For sequence-level collaboration, 
% we adopt Sequence Selection as a baseline.
we compare with Sequence Selection, where each expert independently generates a full response using greedy decoding, and an external reward model selects the highest-scoring output.
%
% This approach uses an external reward to evaluate the responses generated by each model after complete generation and selects the one with the highest reward.
%
For the token-level collaboration, we include Collab~\citep{chakraborty2025collab}, 
% which uses a controlled decoding-based approach with external reward to evaluate the candidate tokens. 
which performs controlled decoding by scoring candidate tokens from multiple models with an external reward signal; we follow the original decoding procedure and vary only the reward model to ensure fair comparisons.
%
% For the model merging approach, 
We also include two popular model merging approaches, DARE~\citep{yu2024language} and TaskArithmetic~\citep{ilharco2022editing}. 
%
% Moreover, we include the directly fine-tuned model via SFT and DPO (named Fine-tuned Model in \tabref{table:main}) in our baseline to investigate the impact of the candidate models. 
% Additionally, we include a Fine-tuned Model baseline obtained by directly fine-tuning the base LLM using the same SFT and DPO procedures as \algname, but without any routing or collaboration mechanism, thereby isolating the benefit of token-level multi-LLM collaboration and complementary logit contributions.
Additionally, we include a Fine-tuned Model baseline that applies the same SFT and DPO as \algname but removes routing and collaboration, isolating the contribution of complementary logits.
%
% For our algorithm, we include two variants \algname and \algname-SFT. 
%
% The “\algname-SFT” represents the router trained using only the SFT phase with the loss defined in \eqnref{eq:sftloss}, whereas “FusionRoute” corresponds to our final router trained with both SFT and CDPO.
%

% \zz{
% What is the benefit of including two variants in this main experiment section?
% }

\paragraph{Models.} 
We conduct experiments on both the Llama-3~\citep{dubey2024llama} and Gemma-2~\citep{team2024gemma} families, using the model checkpoints provided by \citet{he2025mergebench}. 
%
% For each family, we select three expert models specializing in mathematics, coding, and instruction following, respectively. 
%
Specifically, for the Llama-3 family, we use math expert models \href{https://huggingface.co/MergeBench/Llama-3.1-8B-Instruct_math}{Llama-3.1-8B-Instruct$\_$math} and coding expert models \href{https://huggingface.co/MergeBench/Llama-3.1-8B-Instruct_coding}{Llama-3.1-8B-Instruct$\_$coding} from MergeBench~\citep{he2025mergebench} as the two expert models, and \href{https://huggingface.co/meta-llama/Llama-3.1-8B-Instruct}{Llama-3.1-8B-Instruct} as the instruction-following expert. 
% \yh{huggingface link?}\zz{good call, let's put these huggingface links all in the appendix?}\nuoya{I add huggingface link here.}. 
%
Following~\citet{chakraborty2025collab}, we use the one open-sourced  \href{https://huggingface.co/Ray2333/reward-model-Mistral-7B-instruct-Unified-Feedback}{Ray2333/reward-model-Mistral-7B-instruct-Unified-Feedback}
as the external reward for Collab~\citep{chakraborty2025collab}. 
% \yh{hf link here}.
%
For the Gemma-2 family, we choose  \href{https://huggingface.co/MergeBench/gemma-2-2b-it_math}{Gemma-2-2B-Instruct\_math}, \href{https://huggingface.co/MergeBench/gemma-2-2b-it_coding}{Gemma-2-2B-Instruct$\_$coding} and \href{https://huggingface.co/MergeBench/gemma-2-2b-it_instruction}{Gemma-2-2B-Instruct$\_$instruction} from MergeBench~\citep{he2025mergebench} as three expert models. 
%
For a fair comparison, we use 
\href{https://huggingface.co/weqweasdas/RM-Gemma-2B}{weqweasdas/RM-Gemma-2B} as the external reward for Collab~\citep{chakraborty2025collab}, instead of a larger 7B reward model.

\paragraph{Implementation and training.}
We randomly select 500 samples from the \href{https://huggingface.co/datasets/mlabonne/open-perfectblend}{PerfectBlend} dataset~\citep{xu2024perfect} as the test set and use the remaining samples as the training pool.
%
For the initial SFT phase, we randomly sample 200k examples from the PerfectBlend training split, which provides a balanced mixture of mathematics, coding, and instruction-following tasks.
% Then, we randomly sample 200k samples from the trained dataset of \texttt{PerfectBlend} dataset for SFT phase, as it is a mixed dataset covering areas such as mathematics, coding, and instruction following. 
%
For both the Llama and Gemma families, 
% the router is fine-tuned from the instruction-following expert by minimizing the loss function \eqnref{eq:sftloss} with $\lambda=1/3$ and learning rate $1\times 10^{-5}$ for one epoch. 
the router is initialized from the instruction-following expert and fine-tuned by minimizing the loss in \eqnref{eq:sftloss} with $\lambda=1/3$ and a learning rate of $10^{-5}$ for one epoch.
%
After obtaining the policy from the SFT phase, 
% we further fine-tune the framework starting from this policy. 
we further train the model using the mixed training procedure in Algorithm~\ref{alg:mixdpo}.
%
% We randomly sample 100k samples in\texttt{PerfectBlend} dataset as $\cD_{\text{SFT}}$ and 100k samples in \texttt{Openhermes} dataset as $\cD_{\text{DPO}}$ in Algorithm~\ref{alg:mixdpo}, with learning rate $1\times 10^{-5}$, $\beta=0.1$ and $\lambda=1/3$ for one epoch.
%
Specifically, we sample 100k examples from the PerfectBlend training split as $\cD_{\text{SFT}}$ and 100k preference pairs from the \href{https://huggingface.co/datasets/argilla/OpenHermesPreferences}{OpenHermes} dataset~\citep{OpenHermes_2.5} as $\cD_{\text{DPO}}$ with learning rate  $10^{-5}$, $\beta=0.1$, and $\lambda=1/3$ for one epoch.
%
For the directly fine-tuned baseline, we apply the same SFT and DPO procedures and hyperparameters, but without training the routing linear layer.
%
For model merging baselines, we use the default parameters $p=0.9$ and $\lambda=1$ for DARE~\citep{yu2024language} and $\lambda=1$ for TaskArithmetic~\citep{ilharco2022editing}. 
%
% The three models are open-sourced model based on Llama3.1-8B-Instruct, with different expertise. 

% \centerline{\begin{tabular}{|c|c|c|c|}
% \hline
%  & GSM8K & MBPP & OpenInstruct \\
% \hline
% Math Expert & \textbf{83.5\%} & 7.46 & 5.70 \\
% \hline
% Code Expert & 29.5\% & \textbf{16.20} & 10.07 \\
% \hline
% Instruction-Following Expert & 55\% & 13.37 & \textbf{12.78} \\
% \hline
% \end{tabular}
% }

% The following table shows the result of different approaches. 


% \centerline{\begin{tabular}{|c|c|c|c|}
% \hline
%  & GSM8K & MBPP & OpenInstruct \\
% \hline
% Math Expert & \textbf{83.5\%} & 7.46 & 5.70 \\
% \hline
% Code Expert & 29.5\% & \textbf{16.20} & 10.07 \\
% \hline
% Instruction-Following Expert & 55\% & 13.37 & \textbf{12.78} \\
% % \hline
% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% % Router with end-to-end training & & & \\

% \hline
% \end{tabular}
% }


% \subsection{Evaluation}
% I try different approaches to combine the router and model. The reward model is chosen as https://huggingface.co/Skywork/Skywork-Reward-V2-Llama-3.1-8B, which is the SOTA reward model in RewardBench2. The training dataset is PerfectBlend, which is a mixed dataset containing Chat, Math, Code and Instruction Following. 3

% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & Reward \\
% \hline
% Math Expert & 8.91\\
% \hline
% Code Expert &  5.71 \\
% \hline
% Instruction-Following Expert & 12.36 \\
% \hline 
% Collab & 13.85\\
% \hline
% Llama3.1-8B-SFT &  12.76  \\
% \hline
% Routing \& Router Selection & 13.63  \\
% \hline
% Routing \& Router Logits Merging & 14.43 \\
% \hline
% Routing without guidance & 12.42 \\
% \hline
% Routing \& Combine Training & 10.76\\
% \hline 
% Routing with Separate Training & 13.57\\
% % \hline
% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% % Router with end-to-end training & & & \\
% \hline
% \end{tabular}
% }


% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & Router Logits Merging's Winrate \\
% \hline
% Math Expert & 60.7\%\\
% \hline
% Code Expert &  82.2\% \\
% \hline
% Instruction-Following Expert & 57.8\% \\
% \hline 
% Collab & 51.9\%\\
% \hline
% Llama3.1-8B-finetune (SFT) &  59.7\%  \\
% \hline
% Routing \& Router Selection & 55.5\% \\
% \hline
% Routing without guidance & 57.3\% \\
% \hline
% Routing \& Combine Training & 67.75\% \\ 
% \hline
% Routing with Separate Training & 56.2\%\\
% \hline

% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }

% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & Router Combine GPT-4o Winrate \\
% \hline 
% Collab & 52.75\%\\
% \hline
% 8B Finetune (SFT) & 57\% \\
% \hline


% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }

% % \centerline{\begin{tabular}{|c|c|c|c|c|c|}
% % \hline
% %  & GSM8K & MATH & MBPP & Humaneval & IfEval \\
% %  \hline
% %  Router Combine & 82.75\% & 30\% & 34.5\% & 55.48\% & 0.63\\

% % \hline 
% % Collab & 85.25\% & 35.5\% & 22.5\% & 43.9\% & 0.47\\
% % \hline
% % 8B Finetune (SFT) &72.75\% & 30\% & 34\% & 52.43\% & 0.66 \\
% % \hline
% % Math Expert & 84.75\% & 23\% & 13\% & 28.65\%  & 0.26\\
% % \hline
% % Code Expert & 32.25\% & 4.5\% & 30\% & 55.48\% & 0.44 \\
% % \hline
% % Instruct Expert & 71.5\% & 26.5\% & 31.5\% & 51.8\% & 0.67\\
% % \hline 



% % % Collab with General Reward Function & &  &\\
% % % \hline
% % % Router with Expert Label (Which expert) & & & \\
% % % \hline
% % % Router with Mixed Label & & & \\
% % % \hline
% % \end{tabular}
% % }

\subsection{Main Results} \label{sec:exp_crossdomain}

% \paragraph{Cross-Domain Performance.}
\subsubsection{General-purpose Performance with Specialized Experts}
In practical deployment, users interact with a single model without knowing the prompt’s domain. We therefore evaluate \algname in a mixed-domain setting, where it automatically selects the appropriate expert at inference time. 
%
We therefore evaluate \algname in a general-purpose, mixed-domain setting, where the model must automatically leverage the most appropriate expert at inference time, without any manual checkpoint selection.
%
We consider five benchmark datasets covering diverse expert domains: GSM8K~\citep{cobbe2021training} and MATH500~\citep{lightman2023lets} for mathematical reasoning, MBPP~\citep{austin2021program} and HumanEval~\citep{chen2021codex} for code generation, and IfEval~\citep{zhou2023instruction} for instruction following.
%
% To evaluate the multi-facet capability of our models across diverse domains, we consider five benchmark datasets: 
% \begin{itemize}
%     \item \textbf{GSM8K}: A dataset of grade-school math word problems.  
%     \item \textbf{MATH500}: A collection of challenging mathematical problems requiring multi-step reasoning.  
%     \item \textbf{MBPP}: The Python Programming dataset, focusing on code generation tasks.  
%     \item \textbf{HumanEval}: A code generation benchmark with test cases.  
%     \item \textbf{Ifeval}: A set of instruction-following evaluation tasks across multiple domains.  
% \end{itemize}
%
These datasets allow us to measure model performance across math, coding, and instruction-following tasks, providing a comprehensive cross-domain evaluation. 
%
We use greedy decoding as the generation approach, more implementation details for each task are provided in \appref{appendix:sec:generation}. 
% \yh{Shall we put this paragraph to the experimental setup instead of results?}\nuoya{I think it is fine since we have two experiment settings and we introduce one of them here.}
%

% Table~\ref{table:main} summarizes the main experimental results for the Llama-3 and Gemma-2 families.
%
Our results show that both algorithms consistently achieve the highest average performance across the five domains on both two LLM families and get performance comparable to domain-specific experts on individual tasks.
%
\tabref{table:main} summarizes the results on both the Llama-3 and Gemma-2 families. 
% \yh{For this table, maybe we can put the performance of 3 experts into the top of the table and use a line to separate them with the other baselines, only as a reference. By not directly comparing FusionRoute results with the expert results, I think we can bold most of our results.}
%
Across both model families, \algname achieves the highest average performance, consistently outperforming sequence-level collaboration, prior token-level collaboration (Collab), model merging methods, and directly fine-tuned models. 
%
These results demonstrate that \algname effectively functions as a general-purpose model assembled from specialized experts, relieving users from the need to select domain-specific checkpoints while delivering strong and stable performance across heterogeneous tasks. 
%
The examples of routing behavior in several domain-specific tasks are provided in \appref{appendix: router behavvior}.
%

Importantly, \algname does not sacrifice specialization.
%
On benchmarks where a particular expert is expected to perform best---such as math experts on GSM8K~\citep{cobbe2021training} and MATH500~\citep{lightman2023lets} or coding experts on MBPP~\citep{austin2021program} and HumanEval~\citep{chen2021codex}---\algname remains competitive and often matches or exceeds the corresponding expert's performance. 
%
This shows that \algname is compatible with expert specialization, while being substantially more robust and generalized in mixed-domain usage.
%
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{HumanEval} & \textbf{IfEval} & \textbf{Avg Acc.} \\
\midrule
\multicolumn{7}{c}{\textit{Llama-3 Family}} \\
\midrule
\multicolumn{7}{c}{\textit{Expert Models}} \\
Math Expert      & 0.86 & 0.36 & 0.23 & 0.37 & 0.31 & 0.426 \\
Code Expert      & 0.52 & 0.15 & 0.34 & 0.66 & 0.48 & 0.430 \\
Instruct Expert  & 0.74 & 0.27 & 0.36 & 0.52 & 0.67 & 0.512 \\
\midrule
\multicolumn{7}{c}{\textit{Collaboration Approaches}} \\
% FusionRoute-OnlySFT (ours) & 0.85 & 0.38 & 0.36 & 0.60 & 0.67 & \cellcolor{red!15}\textbf{0.572} \\
% FusionRoute (ours) & 0.82 & 0.33 & 0.36 & 0.63 & 0.69 & \cellcolor{blue!10}\textbf{0.566} \\
Sequence Selection & 0.76 & 0.31 & 0.21 & 0.45 & 0.50 & 0.466 \\
Collab & \underline{0.82} & \underline{0.32} & 0.28 & 0.54 & 0.55 & 0.502 \\
Fine-tuned Model & 0.75 & 0.26 & \underline{0.36} & \underline{0.58} & \textbf{0.72} & \underline{0.536} \\
DARE & 0.75 & 0.28 & 0.23 & 0.26 & 0.32 & 0.368 \\
TaskArithmetic & 0.82 & 0.32 & 0.24 & 0.39 & 0.35 & 0.424 \\
% Math Expert & \textbf{0.86} & \textbf{0.36} & 0.23 & 0.37 & 0.31 & 0.426 \\
% Code Expert & 0.52 & 0.15 & 0.34 & \textbf{0.66} & 0.48 & 0.430 \\
% Instruct Expert & 0.74 & 0.27 & 0.36 & 0.52 & 0.67 & 0.512 \\
\rowcolor{blue!10}\algname (ours) & \textbf{0.82} & \textbf{0.33} & \textbf{0.36} & \textbf{0.63} & \underline{0.69} & \textbf{0.566} \\
\midrule
\midrule
\multicolumn{7}{c}{\textit{Gemma-2 Family}} \\
\midrule
\multicolumn{7}{c}{\textit{Expert Models}} \\
Math Expert & 0.67 & 0.27 & 0.22 & 0.36 & 0.47 & 0.398 \\
Code Expert & 0.39 & 0.16 & 0.27 & 0.41 & 0.52 & 0.350 \\
Instruction Expert & 0.19 & 0.08 & 0.23 & 0.34 & 0.61 & 0.290 \\
\midrule
\multicolumn{7}{c}{\textit{Collaboration Approaches}} \\
% FusionRoute-OnlySFT (ours) & 0.64 & 0.23 & 0.25 & 0.41 & 0.62 & \cellcolor{blue!10}\textbf{0.430} \\
% FusionRoute (ours) & 0.65 & 0.22 & 0.25 & 0.40 & 0.61 & \cellcolor{red!15}\textbf{0.426} \\
Sequence Selection & \underline{0.62} & \textbf{0.24} & \textbf{0.27} & \underline{0.37} & 0.54 & \underline{0.408} \\
Collab & 0.52 & 0.22 & \underline{0.26} & 0.35 & 0.45 & 0.360 \\
Fine-tuned Model & 0.54 & 0.17 & 0.24 & 0.34 & \textbf{0.68} & 0.394 \\
TaskArithmetic & 0.43 & 0.15 & 0.14 & 0.28 & 0.34 & 0.268 \\
DARE & 0.36 & 0.10 & 0.14 & 0.16 & 0.36 & 0.224 \\
% Math Expert & \textbf{0.67} & \textbf{0.27} & 0.22 & 0.36 & 0.47 & 0.398 \\
% Code Expert & 0.39 & 0.16 & \textbf{0.27} & \textbf{0.41} & 0.52 & 0.350 \\
% Instruction Expert & 0.19 & 0.08 & 0.23 & 0.34 & 0.61 & 0.290 \\
\rowcolor{blue!10}\algname (ours) & \textbf{0.65} & \underline{0.22} & 0.25 & \textbf{0.40} & \underline{0.61} & \textbf{0.426} \\
\bottomrule
\end{tabular}
\caption{
    Cross-domain performance comparison on Llama-3 and Gemma-2 families. 
    %
    Best and second-best performance within each family are highlighted by \textbf{bold} and \underline{underline}, respectively.
    %
}
\label{table:main}
\end{table*}
%






% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & DPO (model) + SFT (linear) Winrate \\
% \hline
% Math Expert & 69.5\%\\
% \hline
% Code Expert &  77.5\% \\
% \hline
% Instruction-Following Expert & 84.5\% \\
% \hline 
% Collab & 63\%\\
% \hline
% 8B-finetune (DPO) &  55.5\%  \\
% \hline
% 3B-finetune (DPO) & 62\% \\
% \hline
% DPO(model) + DPO(linear) & 57\% \\
% \hline
% \makecell{DPO(model) + SFT(linear) \\ (separated)} & 56.7\% \\ 
% \hline
% \makecell{DPO(model) + DPO(linear)\\(separated)} & 61.5\%\\
% \hline
% \makecell{ARM(model) + SFT(linear)} & 62\%\\
% \hline

% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }

% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & Average Reward \\
% \hline
% Math Expert & 12.71\\
% \hline
% Code Expert &  13.33 \\
% \hline
% Instruction-Following Expert & 7.32 \\
% \hline 
% Collab & 16.59\\
% \hline
% 8B-finetune (DPO) &  17.00  \\
% \hline
% 3B-finetune (DPO) & 16.25 \\
% \hline
% SFT(model) + DPO(linear) & 19.14 \\
% \hline
% DPO(model) + DPO(linear) & 18.15 \\
% \hline
% \makecell{DPO(model) + SFT(linear) \\ (separated)} & 19.32 \\ 
% \hline
% \makecell{DPO(model) + DPO(linear)\\(separated)} & 17.58\\
% \hline

% \makecell{ARM(model) + SFT(linear)} & 17.48\\
% \hline

% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }


% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & DPO (model) + SFT (linear) GPT-4o Winrate \\
% \hline 
% Collab & 62\%\\
% \hline
% 8B-finetune (DPO) &  55\%  \\
% \hline
% 3B-finetune (DPO) & 57\% \\
% \hline


% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }






% \centerline{\begin{tabular}{|c|c|c|c|c|c|}
% \hline
%  & GSM8K & MATH & MBPP & Humaneval & IfEval \\
%  \hline
%  Router Combine (3B Router) & 79\% & 32.5\% & 29.5\% & 62.8\% & 0.68\\
%   \hline
%  Only Model (3B Router) & 73\% & 23.5\% & 27\%  & 60.97\% & 0.62\\

% \hline 
%  Router Combine (8B Router) & 78.75\% & 25.5\% (?)  & 33\% & 63.4\% & 0.72\\
%  \hline 
% Only Model (8B Router) & 66.5\% &   & & 57.3\%  & 0.64 \\

%  \hline
%  (Only SFT) Router Combine (3B Router) & 79.25\% & 32\% & 29\% & 61.58\% & 0.66\\
%   \hline
%  (Only SFT) Only Model (3B Router) & 83\% & 35\% & 25.5\% & 61.58\% &0.62\\

% \hline 
%  (Only SFT) Router Combine (8B Router)  & 85.25\% & 32.5\% & 32.5\% & 59.75\% &\\
%  \hline 
% (Only SFT) Only Model (8B Router)  & 82\% & 30\% & 28\% &56.7\% & 0.65\\

%  \hline 
%  3B Specific Model  & 85.5\% & 38.5\% & 29\% &62.19\% & \\
%  \hline 
%  8B Specific Model  & 86.5\% & 40.5\% & 32.5\% &64.63\% & \\

%   \hline 
%  (Only SFT) 8B Specific Model  & 86\% & 34.5\% & 32.5\% &62.19\% & \\
%  \hline 
%  (Only SFT) 3B Specific Model  & 85.5\% & 39\% & 28.5\% &60.36\% & \\

% \hline 
% Collab & 82.25\% & 38.5\% & 25.5\% & 53.65\% &0.55\\
% \hline
% 3B Finetune (SFT+DPO) &67.25\% & 35\% & 30\% & 50.6\% &  0.69\\
% \hline
% 8B Finetune (SFT+DPO) &75\% & 30.5\% & 36\% & 57.9\% &  0.72\\
% \hline
% Math Expert & 85.75\% & 39\% & 20.5\% & 36.5\% & 0.31 \\
% \hline
% Code Expert & 52\% & 1\% & 30.5\%  & 66.4\% & 0.48  \\
% \hline
% Instruct Expert & 74.25\% & 26\% & 31.5\% & 51.8\% & 0.67\\
% \hline 



% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }

% \begin{table}[t]
% \centering
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg\\
% \midrule
% FusionRoute-OnlySFT (ours) & 0.85 & 0.38 & 0.36 & 0.60 & 0.67 & \cellcolor{red!15}\textbf{0.572} \\
% FusionRoute (ours) & 0.82 & 0.33 & 0.36 & 0.63 & 0.69 & \cellcolor{blue!10}\textbf{0.566} \\
% Sequence Selection & 0.76 & 0.31 & 0.21 & 0.45 & 0.50 & 0.466 \\
% Collab & 0.82 & 0.32 & 0.28 & 0.54 & 0.55 & 0.502 \\
% Fine-tuned Model & 0.75 & 0.26 & 0.37 & 0.58 & 0.72 & 0.536 \\
% DARE & 0.75 & 0.28 & 0.23 & 0.26 & 0.32 & 0.368 \\
% TaskArithmetic & 0.82 & 0.32 & 0.24 & 0.39 & 0.35 & 0.424 \\
% Math Expert & 0.86 & 0.36 & 0.23 & 0.37 & 0.31 & 0.426 \\
% Code Expert & 0.52 & 0.15 & 0.34 & 0.66 & 0.48 & 0.430 \\
% Instruct Expert & 0.74 & 0.27 & 0.36 & 0.52 & 0.67 & 0.512 \\
% \bottomrule
% \end{tabular}
% \caption{Llama-3 Family}
% \end{subtable}
% \\ \vspace{1em}
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg\\
% \midrule
% % Collab & 58.25 & 21.6 & 26.4 & 35.3 & 48.95 & 0.382 \\
% FusionRoute-OnlySFT (ours) & 0.64 & 0.23 & 0.25 & 0.41 & 0.62 & \cellcolor{blue!10}\textbf{0.430} \\
% % SFT DPO Mix Training & 64.75 & 23.0 & 24.6 & 41.4 & 59.23 & 0.427 \\
% FusionRoute (ours) & 0.65 & 0.22 & 0.25 & 0.40 & 0.61 & \cellcolor{red!15}\textbf{0.426} \\
% Sequence Selection & 0.62 & 0.24 & 0.27 & 0.37 & 0.54 & 0.408 \\
% Collab & 0.52 & 0.22 & 0.26 & 0.35 & 0.45 & 0.360 \\
% Fine-tuned Model & 0.54 & 0.17 & 0.24 & 0.34 & 0.68 & 0.394 \\
% TaskArithmetic & 0.43 & 0.15 & 0.14 & 0.28 & 0.34 & 0.268 \\
% DARE & 0.36 & 0.10 & 0.14 & 0.16 & 0.36 & 0.224 \\
% Math Expert & 0.67 & 0.27 & 0.22 & 0.36 & 0.47 & 0.398 \\
% Code Expert & 0.39 & 0.16 & 0.27 & 0.41 & 0.52 & 0.350 \\
% Instruction Expert & 0.19 & 0.08 & 0.23 & 0.34 & 0.61 & 0.290 \\
% \bottomrule
% \end{tabular}
% \caption{Gemma-2 Family}
% \end{subtable}
% \caption{Performance comparison for several benchmarks on cross-domain evaluation on Gemma-2 Family. The best and second best are marked with \colorbox{red!15}{red} and \colorbox{blue!10}{blue} colors respectively.}\label{table:main}
% \end{table}



% \centerline{\begin{tabular}{|c|c|c|c|c|c|}
% \hline
%  & GSM8K & MATH500 & MBPP & Humaneval & IfEval \\
% %  Router Combine (3B Router) & 79\% &  & 29.5\% & 62.8\% & 0.68\\
 

% % \hline 
% %  Router Combine (8B Router) & 78.75\% &   & 33\% & 63.4\% & 0.72\\
 


 
% \hline 
%  (Only SFT) Router Combine (8B Router)  & 85.25\% & 37.6\% & 35.8\% & 59.75\% & 0.67\\
% \hline
% SFT + DPO Mix Training (Combine Logits) & 81    .75\% & 32.8\% & 36\% & 63.41\% & 0.69\\
% \hline
% Collab & 82.25\% & 31.6\% & 28.4\% & 53.65\% &0.55\\
% \hline
% SFT+DPO Mix training (8B Router) & 82.25\% & 33\% & 37.4\%  & 60.97\% & 0.71  \\
% \hline
% 8B Finetune (SFT+DPO) &75\% & 26\% & 37\% & 57.9\% &  0.72\\
% \hline
% DARE(p=0.9, $\lambda$=1) &  74.75\% & 28.2\% & 22.8\% & 26.2\%& 0.32\\
% \hline
% DARE(p=0.5, $\lambda$=0.5) & 87.25\% & 34.8\% & 33.6\% & 60.97\% & 0.49\\
% \hline
% TIES(k=0.2, $\lambda$=1) &  89.5\% & 35\% & 31.8\% & 60.97\%& 0.57\\
% \hline
% TaskArithmetic($\lambda$=1) &  82\% & 31.8\% & 24\% & 39.02\%& 0.35\\
% \hline
% Math Expert & 85.75\% & 36.4\% & 22.8\% & 36.5\% & 0.31 \\
% \hline
% Code Expert & 52\% & 14.8\% & 33.8\%  & 66.4\% & 0.48  \\
% \hline
% Instruct Expert & 74.25\% & 26.8\% & 36.4\% & 51.8\% & 0.67\\
% \hline 



% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }



% \begin{figure}[t]
% \setlength{\abovecaptionskip}{2pt}
%     \centering
%     \begin{subfigure}{\linewidth}
%     \centering
%     \begin{subfigure}{0.45\linewidth}
%         \includegraphics[width=\linewidth]{figures/winratellama3.png}
%         \caption{Llama3 Family}
%         \label{fig:placeholder}
%     \end{subfigure}
%     \begin{subfigure}{0.45\linewidth}
%         \includegraphics[width=\linewidth]{figures/winrategemma2.png}
%         \caption{Gemma 2 Family}\label{fig:placeholder_congestiongames}
        
%     \end{subfigure}
%     \end{subfigure}
    
    
%     \caption{GPT-4o winrate on general datasets compared to fine-tuned model.}
% \end{figure}
% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & GPT-4o Winrate compared to 8B Finetune (SFT + DPO)\\
% \hline 
% Collab & 44.35\% \\
% \hline
% (Only SFT) Router Combine (8B Router) &  58.55\% \\
% \hline
% SFT+DPO Mix Training (8B Router) & 64.65\% \\
% \hline
% SFT+DPO Mix Training (Combine Logits) & 62.1\% \\
% \hline
% DARE(p=0.9, $\lambda$=1) & 37.45\%\\
% \hline
% TaskArithmetic & 44.45\%\\
% \hline

% \end{tabular}
% }

% \subsection{Qwen2.5}


% \centerline{\begin{tabular}{|c|c|c|c|c|c|}
% \hline
%  & GSM8K & MATH500 & MBPP & Humaneval & IfEval \\
% %  Router Combine (3B Router) & 79\% &  & 29.5\% & 62.8\% & 0.68\\
%  \hline
% Collab & 59.5\% & 24.4\% & 39.2\% & 32.92\% & \\
% \hline
% Router Combine &  & 33\% & 46.4\% &41.4\%  & \\
% \hline 
% Finetune & 31.25\% &  18\% & 30.4\%& 3\%(?)& \\
 
% \hline
% Math Expert & 85\% & 29.8\% & 28.4\% & 29.27\% & 0.34\\
% \hline
% Code Expert & 76\% & 29\% & 41.4\%  & 62.2\% & 0.70\\
% \hline
% Instruct Expert & 30.25\% & 18.4\% & 36.4\% & 38.4\% &0.72 \\
% \hline 



% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }

% We can see the result of Qwen2.5 are very strange. Actually, the fine-tuned model just does not follow the rule of generating the code and make our code extraction fail.



% Collab with General Reward Function & &  &\\
% \hline
% Router with Expert Label (Which expert) & & & \\
% \hline
% Router with Mixed Label & & & \\
% \hline

% \centerline{\begin{tabular}{|c|c|c|c|c|c|}
% \hline
%  & GSM8K & MATH500 & MBPP & Humaneval & IfEval \\
% %  Router Combine (3B Router) & 79\% &  & 29.5\% & 62.8\% & 0.68\\
%  \hline
% Collab & 58.25\% & 21.4\% & 27\% & 34.75\% & 48.9\\
% \hline
% Router Combine & 63.5\% & 22.2\% & 24.6\% & 39.63\% & 54.5\\
% \hline
% SFT DPO Mix Training & 65\% & 22\% & 25.2\% &38.4\%  & 55.2\\
% \hline 
% Finetune (SFT+DPO) & 55\% &  19.2\% & 27.4\%& 32.9\%& 57.3 \\

%  \hline
% DARE & 54.25\% & 17.8\% &19.2\% &30.4\% & 34.6\\
% \hline
% TaskArithmetic & 57.75\% &18.8\% & 22.2\% & 37.1\% &35.1\\
% \hline
% Math Expert & 66.5\% & 27.4\% & 21.8\% & 35.9\% & 47.2 \\
% \hline
% Code Expert & 39.25\% & 15.6\% & 27.2\%  & 41.4\% & 51.9 \\
% \hline
% Instruct Expert & 60.5\% & 16.4\% & 27.2\% & 37.8\% & 60.8\\
% \hline 



% % Collab with General Reward Function & &  &\\
% % \hline
% % Router with Expert Label (Which expert) & & & \\
% % \hline
% % Router with Mixed Label & & & \\
% % \hline
% \end{tabular}
% }







% \begin{table}[H]
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg\\
% \midrule
% % Collab & 58.25 & 21.6 & 26.4 & 35.3 & 48.95 & 0.382 \\
% SFT (ours) & 63.75 & 22.6 & 24.6 & 40.8 & 62.19 & \cellcolor{blue!10}\textbf{0.429} \\
% % SFT DPO Mix Training & 64.75 & 23.0 & 24.6 & 41.4 & 59.23 & 0.427 \\
% SFT+CDPO (ours) & 65.0 & 21.6 & 25.0 & 40.2 & 61.49 & \cellcolor{red!15}\textbf{0.426} \\
% Collab & 51.5 & 21.6 & 25.6 & 34.75 & 44.59 & 0.357 \\
% Fine-tuned Model & 54.0 & 16.8 & 24.4 & 31.7 & 67.59 & 0.389 \\
% TaskArithmetic & 42.5 & 15.4 & 14.2 & 28.4 & 34.49 & 0.271 \\
% DARE & 35.5 & 10.4 & 14.2 & 16.4 & 35.54 & 0.224 \\
% Math Expert & 66.5 & 27.4 & 21.8 & 35.9 & 47.2 & 0.398 \\
% Code Expert & 39.25 & 15.6 & 27.2 & 41.4 & 51.9 & 0.351 \\
% Instruction Expert & 19.0 & 7.8 & 23.4 & 34.1 & 60.62 & 0.291 \\
% \bottomrule
% \end{tabular}
% \caption{Performance comparison for several benchmarks on cross-domain evaluation on Gemma-2 Family. The best and second best are marked with \colorbox{red!15}{red} and \colorbox{blue!10}{blue} colors respectively.}
% \end{table}

\subsubsection{Performance on General Dataset}
%
\begin{figure}[H]
\setlength{\abovecaptionskip}{2pt}
    \centering
    \begin{subfigure}{\linewidth}
    \centering
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/llama_performance.png}
        \caption{Llama3-8B Family}
        \label{fig:placeholder}
    \end{subfigure}
    \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{figures/gemma_performance.png}
        \caption{Gemma2-2B  Family}\label{fig:placeholder_congestiongames}
        
    \end{subfigure}
    \end{subfigure}
    \caption{
    GPT-4o winrate on general datasets compared to fine-tuned model.
    %
    % \zz{make the legends, labels even bigger? Also no need for the matplotlib titles since we have them in latex. Also preferably not use similar blue for both DARE and Collab since they are very different methods in different categories}
    }\label{fig:winrate}
\end{figure}
%
% To test the general performance of FusionRoute without specific domain, we use 500 prompts from testing dataset of \texttt{PerfectBlend} to generate responses for each algorithm, within 300 max token. 
To further assess overall response quality beyond task-specific correctness, we evaluate \algname on a held-out general dataset using pairwise comparisons.
%
Specifically, we sample 500 prompts from the PerfectBlend~\citep{xu2024perfect} test set and generate responses with a maximum length of 300 tokens.
%
Then, we use GPT-4o to evaluate the overall response quality compared to the response of the directly fine-tuned model (Fine-tuned Model in \tabref{table:main}). 
%
For two responses, the pairwise comparison is selected from \textit{win}, \textit{tie} and \textit{loss}, and the win rate is computed as the proportion of wins, with ties counted as half a win, over 500 evaluation examples.
%
Addition details such as evaluation prompt provided in \appref{appendix:sec:generation}. 
%
As shown in \figref{fig:winrate}, \algname achieves a substantially higher win rate than the fine-tuned baseline on both model families, indicating improved overall response quality on general prompts. 
%
This improvement reflects better alignment, fluency, and formatting, complementing the strong task-level performance observed on domain benchmarks.
%

% \subsection{Discussion}

\subsubsection{\algname is More Beneficial at a Larger Scale} 
% \yh{Given two models, shall we use this observation as a conclusion in the title?}
As shown in \figref{fig:winrate}, the performance gap between \algname and other baselines becomes markedly larger in the 8B Llama-3 family. 
%
In this setting, both existing token-level collaboration (Collab~\citep{chakraborty2025collab}) and sequence-level selection exhibit substantial degradation in win rate, whereas \algname continues to improve response quality. 
%
This suggests that as model capacity increases, purely selecting among fixed expert outputs becomes increasingly brittle, while \algname's complementary routing mechanism is able to effectively leverage the additional representational capacity to refine and correct expert predictions.
%

In contrast, in the 2B Gemma-2 family, the gap between \algname and pure token-level collaboration is smaller.
%
While expert-only token-level collaboration still under-performs \algname, it remains competitive and even outperforms the directly fine-tuned baseline. 
%
This indicates that at smaller scales, expert models alone can already capture a reasonable portion of the desired behavior, leaving less room for complementary correction. 
%
Overall, these results suggest that router-based complementary generation becomes increasingly important as model scale grows, whereas expert-only token-level collaboration may suffice in more capacity-constrained settings.
% As shown in \figref{fig:winrate}, the performance gap between \algname and other baselines widens for the larger 8B models, where the existing token-level collaboration method Collab~\citep{chakraborty2025collab} and sequence-level selection perform both notably poorly. 
%
% In the smaller 2B family, pure token-level collaboration still under-performs compared to \algname, but the gap is narrower, and it also performs better than the directly fine-tuned model. 
%
% These results indicate that incorporating the router's complementary logits in the final generation is particularly beneficial for larger LLMs, whereas pure token-level collaboration that selects the next token only among candidate models can still provide reasonable performance in smaller-scale settings.
%






% \begin{table}[H]
% \centering
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg & Winrate \\
% \midrule
% Sequence Selection & 0.76 & 0.31 & 0.21 & 0.45 & 0.50 & 0.466 & 0.563\\
% \algname & 0.82 & 0.33 & 0.36 & 0.63 & 0.69 & \textbf{0.566} & 0.621 \\
% \bottomrule
% \end{tabular}
% \caption{Llama-3 Family}
% \end{subtable}
% \\ \vspace{1em}
% \begin{subtable}{0.9\linewidth}
% \centering
% \small
% \setlength{\tabcolsep}{8pt}
% \renewcommand{\arraystretch}{1.15}
% \begin{tabular}{lccccccc}
% \toprule
% \textbf{Method} & \textbf{GSM8K} & \textbf{MATH500} & \textbf{MBPP} & \textbf{Humaneval} & \textbf{IfEval} & Avg & Winrate \\
% \midrule
% % Collab & 58.25 & 21.6 & 26.4 & 35.3 & 48.95 & 0.382 \\
% Sequence Selection & 0.62 & 0.24 & 0.27 & 0.37 & 0.54 & 0.408 & 0.561 \\
% % SFT DPO Mix Training & 64.75 & 23.0 & 24.6 & 41.4 & 59.23 & 0.427 \\
% \algname & 0.65 & 0.22 & 0.25 & 0.40 & 0.61 & \textbf{0.426} & 0.5745 \\
% \bottomrule
% \end{tabular}
% \caption{Gemma-2 Family}
% \end{subtable}
% \caption{Cross-domain performance of purely token-level routing and \algname. }\label{table:ablation pms}
% \end{table}




% \textbf{Comparison with Sequence-Level Collaboration}
% \centerline{\begin{tabular}{|c|c|}
% \hline
%  & GPT-4o Winrate compared to Finetune (SFT + DPO)\\
% \hline 
% Collab (7B RM) & 57.5\% \\
% \hline 
% Collab (2B RM) & 52.35\% \\
% \hline
% Router Combine & 54.35\% \\
% \hline
% SFT+DPO Mix Training & 56.8\% \\
% \hline
% SFT+DPO Mix Training (Combine Logits) & 57.45\% \\
% \hline
% DARE(p=0.9, $\lambda$=1) & 35.1\% \\
% \hline
% TaskArimetic & 48.1\% \\
% \hline

% \end{tabular}
% }



% \textbf{Collab (7B RM)}
% We let each LLM generate $1$ candidate token and generate next $5$ tokens, and evaluate it using the reward model.
% \textbf{Llama3.1-8B-Finetune}
% We use SFT to fine-tune the base model Llama3.1-8B-Instruct on the Perfectblend training dataset, for 1 epoch and learning rate $1e-5.$
% \textbf{Routing \& Router Selection}
% We use a router to first select the model with the highest routing weight. The selected model then generates its top 5 candidate tokens. Finally, among these candidates, we choose the next token based on the highest router logit score.
% \textbf{Routing \& Router Logits Merging}
% Instead of selecting the top 5 tokens and then choosing the one with the highest router logit, we combine the logits from the selected model and the router, and apply a greedy decoding strategy.
% \textbf{Router Performance}
% We also evaluate the router's performance since it is a trained auto-regressive language model.
% \section{Ablation Study}
% We evaluate the performance when the router selects the best model but does not further guide the next-token generation.

% \section{Router Behavior}

% The red color represents the math agent, blue color represents the code agent, and the green color represents the instruction-following agent. 

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=0.5\linewidth]{histogram.png}
% %     \caption{Agent Distribution}
% %     \label{fig:agentdistribution}
% % \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{model_index_colored_math.png}
%     \caption{Math Problem Example}
%     \label{fig:math}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{model_index_colored_code.png}
%     \caption{Code Problem Example}
%     \label{fig:code}
% \end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{model_index_colored_instruction.png}
%     \caption{Instruction-Following Problem Example}
%     \label{fig:instruction}
% \end{figure}



% \section{DPO Combine Training}
% One candidate approach is to train the combined logits of the router logits and the candidate model logits. We have shown that involving combined logits in the SFT stage does not give a good performance. Now we can try to involve combined logits in DPO stage, since the combined logits in DPO loss will be more natural. 

% In fact, suppose the base model of the router model is  $\pi_{\theta}$. Denote $\log \pi_{final}=\log \pi_{\theta}  + \log \pi_{model}$ 
% we can introduce the complement DPO loss as 
% \begin{align*}
%     L(\pi_{\theta}, \pi_{ref})=-\mathbb{E}_{x,y_w, y_l \in \mathcal{D}}\left[\log \sigma \left(\sum_{t\ge 0}\beta \log \frac{\pi_{final}(y_{t+1}\mid y_{w\le t},  x)}{\pi_{ref}(y_{t+1}\mid y_{w,\le t}, x)}-\beta \log \frac{\pi_{final}(y_{t+1}\mid y_{l, \le t} x)}{\pi_{ref}(y_{t+1}\mid y_{l, \le t} x)}\right)\right]
% \end{align*}


% \section{Theory}

% \subsection{Why the router training approach is better than Collab for token-level collaboration?}

% In this section, we will analyze why our router training approach can achieve a better token-level multi-agent collaboration compared to Collab. 

% We regard the token-level collaboration as an RL process. The state at step $h$ is $s_h = x, y_{\le h}$ and the action $a \in [M]$ represents the selection of the models, where $M$ is the number of the candidate models. Then, the state transits to $s_{h+1}=[x,y_{\le h+1}]$, where $y_{h+1}\sim \pi_{a}(\cdot \mid x,y_{\le t})$.

% We also assume that the optimal next-token generation policy is $\pi^*(\cdot \mid x,y_{\le t})$. Hence, the optimal token for step $h$ is $\pi(y_{h+1}\mid x,y_{\le t})=\arg \max_{\pi^*}[Q_h^{\pi^*}(x,y_{\le t+1})]$. Here, the Q-function is defined by 
% \begin{align*}
%     Q_h^{\pi^*}(x,y_{\le t+1}) = \mathbb{E}_{\pi^*}\left[\sum_{t'=t}^{H}r(x,y_{\le t'+1})\mid x,y_{t+1}\right].
% \end{align*}
% Hence, to make our trajectory close to the $\pi^*$, the ideal action is to choose $a_h \in [M]$ such that $$a_h = \arg\max_{a_h}\mathbb{E}_{y_{t+1}\sim \pi_{a_h}(\cdot \mid x,y_{\le t})}[Q_h^{\pi^*}(x,y_{\le t+1})].$$ 

% Ideally, since we trained on the SFT dataset, the router will return exactly $a_h$ that maximizes the Q-function. Hence, we can derive the total gap between the optimal policy and our router-training approach. Compared to the sentence-level approach, we can achieve a smaller distance between the optimal reward and our derived reward. 

% Then we can use Performance Difference Lemma to bound the total error. In fact, since $a_h = \arg\max_{a_h}\mathbb{E}_{y_{t+1}\sim \pi_{a_h}(\cdot \mid x,y_{\le t})}[Q_h^{\pi^*}(x,y_{\le t+1})]$, we can assume for any $x, y_{\le t}$, there exists a $a \in [M]$ such that $$\Big|\mathbb{E}_{y_{t+1}\sim \pi_{a}(\cdot \mid x,y_{\le t})}[Q_h^{\pi^*}(x,y_{\le t+1})]-\mathbb{E}_{y_{t+1}\sim \pi^*(\cdot \mid x,y_{\le t})}[Q_h^{\pi^*}(x,y_{\le t+1})]\Big| \le \Delta,$$
% where $\Delta$ represents the error between the optimal policy and the candidate model. Hence, we can find 

% \begin{align*}V^{\pi^*}(s_0) - V^{\pi}(s_0) &= \sum_{h=0}^{H-1}\mathbb{E}_{s_h, a_h \sim \mathbb{P}_h^{\pi}(\cdot, \cdot \mid s_0)}\left[Q_h^{\pi^*}(s_h,a_h) -V_h^{\pi^*}(s) \right]\\
% &\le \sum_{h=0}^{H-1} \Delta = H\Delta.\end{align*}

% However, Collab does not try to choose to maximize the Q-function. Instead, the action selection is defined by 
% $$a_h  = \arg\max_{a_h}\mathbb{E}_{y_{t+1}\sim \pi_{a_h}(\cdot \mid x, y_{\le t})}[Q_h^{\pi_{a_h}}(x, y_{\le t+1})].$$

% We can construct an example to show that this can lead to very bad performance. In fact, suppose the optimal actions are $\pi^* = \pi_{a_1}$ for $t \le H/2$ and $\pi^* = \pi_{a_2}$ for $t \ge H/2+1$, the Collab fails to find the optimal policy. 

% \subsection{Why we need router to guide?}
% In the previous subsection, we know that the router training can give us the ideal action if the accuracy for the router is 100\%. However, when the router chooses the wrong model, it can deviate the optimal trajectory and finally fail. Hence, we also fine-tune the base model of the router to get an approximation $\pi_{router}.$ Now, instead of choosing $y_{t+1}\sim \pi_{a_h}(\cdot \mid x,y_{\le t})$, the logits of $y_{t+1}$ becomes 
% $$y_{t+1}=\arg\max_{y}\log \pi_{a_h}(y\mid x, y_{\le t}) + \log \pi_{router}(y\mid x,y_{\le t}).$$ This looks like pulling the trajectory back a bit to align with the optimal policy $\pi^*$.







% % \section{Multi-Objective Optimization}

% % In this section, we discuss how to encourage collaboration among multiple agents in a multi-objective setting. Suppose we have several agents, each optimized for different objectives such as helpfulness and harmlessness. Our goal is to combine these agents with different weights, to generate responses that achieve a good Pareto frontier, effectively balancing the trade-offs between their respective objectives.

% % Previous multi-objective algorithms, such as GenARM and MOD, typically fix a weight vector and generate the final response by combining the agents’ logits using these fixed weights. However, this approach lacks flexibility, as it assumes a constant trade-off across all tokens. In practice, the optimal weighting can vary at each decoding step, and adaptively adjusting the weights token-by-token may lead to better overall responses.

% % Suppose we get $N$ agents $M_1, \cdots, M_N$ and $N$ normalized reward models $R_1,\cdots, R_N$. Previous algorithms always combine $N$ models as 
% % $$\textbf{Logits} = \sum_{i=1}^N \alpha_i \textbf{Logits}(M_i).$$
% % However, it is worth studying that whether it is beneficial to design adaptive weight. To be more specific, at the step $y_{\le t}, $ we can evaluate the objectives' score by the log-likelihood $$R_N(x,y_{\le t})=\sum_{i=1}^{t-1}\log \pi(y_{i}\mid x,y_{i-1}).$$ Then we can use these reward to decide the weight of linearly combining the models.
% % For two models, we use 
% % $$\alpha_t = \gamma \cdot \text{softmax}(-R_N) + (1-\gamma) \cdot [1,0]\  \text{or} \ [0,1]$$ for different $\gamma$ to represent different weights.
% % If $\gamma = 1$, it means that  $\alpha_t = \gamma \cdot \text{softmax}(-R_N)$. In this case, for example, if $N=2$ and objectives are Helpful and Harmless, it means that we assign higher weights for helpful model if the previous response has lower likelihood for helpful model. This provides us an adaptive approach to allocate the weights for the model at the token-level. 

% % \centerline{\includegraphics[scale=0.5]{frontier_with_two_lists.png}}

% % The figure above shows the results for the multi-objective setting. The result shows that our approach can provide better result for max-min goal (maximize the minimum score).



% % % One thing want to try: Use PPO to train the router directly. (Could be applicable for the unknown weight setting, and could be consistent for single-objective and multiple objective?)

==> tex/introduction.tex <==
\section{Introduction}
%

%
Large language models (LLMs) have demonstrated strong performance across an extensive range of tasks, such as mathematical reasoning~\citep{wang2025survey, zhao2025boosting, zhou2025mixture}, code generation~\citep{deng2025swe, huynh2025large, qi2024quantifying, jiang2024survey, jimenez2023swe}, and instruction following~\citep{wang2025beyond, qin2024infobench}. 
%
Although sufficiently large, general-purpose LLMs can often deliver balanced performance across diverse domains~\citep{hurst2024gpt, team2025gemma, yang2025qwen3, zeng2025glm}, their computational and monetary costs make them not ideal for every real-world applications.
%
This motivates an alternative paradigm: employing multiple smaller, specialized LLMs, each excelling in a particular domain while remaining comparatively efficient.
\begin{figure}
%  \vspace{-0.27in}
% \begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/5361767044637_.pic.jpg}
    \caption{
    Sequence-level collaboration is coarse and inefficient, while prior token-level methods are unstable. 
    %
    \algname achieves fine-grained, efficient, and robust token-level collaboration through complementary routing.
    %
    % Comparison of collaboration paradigms in multi-model generation. 
    % %
    % Sequence-level collaboration aggregates entire responses, which is coarse and inefficient. 
    % %
    % Previous token-level collaboration use token-wise selection but remains unstable since the next token is fully dependent on the quality of the candidate model. 
    % %
    % Our \algname enables fine-grained, efficient, and robust token-level routing with complementary logits provided by the router.
    % %
    }
    \label{fig:teaser}
% \end{figure}
\end{figure}
%
However, the strengths of such smaller LLMs often remain uneven---an LLM that performs exceptionally well on one task may underperform on others due to inductive biases~\citep{levine2021inductive, si2023measuring} and domain-specific training distributions~\citep{yuan2023revisiting}.
%
As a result, achieving general-purpose performance through a collection of specialized models hinges on developing mechanisms that can robustly coordinate and leverage their complementary expertise, which has emerged as a central challenge in building efficient and broadly capable LLM systems.
%
% As individual LLMs often possess distinct strengths and inductive biases, leveraging off-the-shelf LLMs and enabling effective collaboration among multiple models within alignment frameworks has become increasingly important for building more general, robust, and powerful systems.

% \begin{wrapfigure}{r}{0.45\linewidth}
%     \vspace{-10pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/winrate_ablation.png}
%     \caption{GPT-4o Winrate Comparison}
%     \vspace{-10pt}
% \end{wrapfigure}



A natural direction toward such collaboration is mixture-of-experts (MoE), in which multiple experts are integrated into a unified architecture and trained jointly with a routing network~\citep{zhou2022mixture, xue2024openmoe, jiang2024mixtral, zengs}. 
%
While effective, this framework is expensive and inflexible since it typically needs gradient access to all experts and substantial additional end-to-end training, and it usually requires expert models to have similar structures.
% \zz{I removed saying that MoE requires expert models to have similar structure since our approach also has this constraint.}
% \nuoya{Our works do not require similar structures?}
%
Another line of work aims to combine the strengths of specialized models through
% assign different LLMs specialized roles within 
multi-agent systems (MAS), 
% allowing them to work together in producing higher-quality responses. 
where different LLMs are assigned different roles with the goal of leveraging the best capabilities of each model or agent during generation~\citep{du2023improving, zheng2025thought}.
%
However, without prior knowledge of 
% each model's expertise or failure modes,
which types of questions each model is best suited for, determining how tasks should be allocated in advance becomes inherently challenging. 
%
Moreover, existing MAS~\citep{liu2024groupdebate, liang2024encouraging,ashiga2025ensemble,huang2024ensemble,chen2025harnessing} typically operate at a coarse response level, where each agent independently generates a full response and a final answer is selected, merged or subjected to debate post hoc. 
%
% This limits the potential synergy between models.
This approach is inefficient, as it requires multiple full-sequence generations, and can even degrade performance when more agents and discussions are involved due to the heavily increased context length~\citep{zheng2025thought}.
%
A third direction is model merging~\citep{yang2024model, he2025mergebench}, which combines multiple specialized models into a single set of parameters.
%
Although training-free and architecturally simple, model merging is often sensitive to hyperparameters and suffers from parameter interference, where the merged weights degrade each model’s specialized capabilities, making it unable to adaptively emphasize different expert behaviors in changing scenarios.
%
% More recently, existing works propose multi-agent collaboration at the \textit{token-level}, which is a more fine-grained and dynamic approach without further training on expert models.
%
% It enables multiple LLM agents to collaborate at the token level during generation, allowing each agent to contribute contextually where its expertise is the most relevant. 

To overcome these limitations, recent work has explored \textit{token-level} multi-agent collaboration, a more fine-grained and dynamic paradigm that allows multiple LLMs to jointly produce each token during generation~\cite{chakraborty2025collab}.
%
However, the effectiveness of these works depends heavily on the quality of the underlying models, making them not robust when expert models perform poorly, or the selection strategy is not correct on certain tasks or tokens.
%
% Also, some of previous work relies on ground-truth reward functions to evaluate every possible token at every time step, which could be very inefficient. 
%
% In addition, existing frameworks are typically evaluated only on a few specific domains or solely on general-purpose datasets, leaving their broad effectiveness unclear. 
%
These limitations lead to the following key question:
%

\begin{center}
% \textit{Can we design a robust, efficient and flexible token-level collaboration approach \\that achieves strong performance on both cross-domain and general datasets?}
\textit{
Can we develop a token-level collaboration paradigm that \\ works robustly, efficiently, and automatically across all scenarios?
}
\end{center}

% Collab proposes a mixture-of-agents controlled decoding algorithm for LLM alignment, where multiple specialized off-the-shelf LLMs (agents), each aligned to different objectives, are dynamically switched at each token during inference based on a long-term utility (Q-function) to maximize alignment with a target reward. Figure 1 shows an example of Collab, where different agents (e.g., a general chat agent and a domain expert) are coordinated at the word/phrase level to produce an optimal, coherent response that neither could achieve alone.


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figure1.jpg}
%     \caption{Illustration of Collab: at each word or phrase, the system dynamically switches between specialized LLM agents (e.g., ChatAgent and Chemical-Expert), enabling collaborative response generation that integrates the strengths of each agent for a more complete and contextually appropriate answer.
% }
%     \label{fig:enter-label}
% \end{figure}

To address this question, we propose \textbf{\algname}, a token-level collaboration framework that unifies \textit{expert selection} and \textit{knowledge complementation} within a single, lightweight router LLM.
%
\algname learns to identify which specialized model is most suitable for generation each next token, enabling fine-grained, context-dependent use of expert capabilities without requiring expensive joint training or per-token evaluation across multiple models~\citep{zhou2022mixture}.
%
At the same time, \algname is trained to provide its own \textit{complementary} generation signal, allowing it to refine or correct an expert whenever the expert is uncertain or unreliable.
%
By fusing the router's corrective logits with those of the selected expert during decoding, \algname achieves both robustness by mitigating expert failures, and efficiency through avoiding the overhead that limits prior multi-LLM collaboration methods.
%
This dual design allows \algname to function as an automatic, domain-agnostic coordination mechanism, enabling consistent performance improvements across diverse tasks and datasets.
%
% To address this question, we train a token-level router model equipped with two key capabilities. 
% %
% First, the router predicts an index corresponding to the expert model most suitable for generating the next token, conditioned on the previously generated text. 
% %
% This design is highly efficient, as it avoids the inference overhead of generating candidate tokens or full responses across multiple models~\citep{chakraborty2025collab}, and it eliminates the significant additional training cost required for jointly training experts in MoE frameworks~\citep{zhou2022mixture}. 
% %
% Second, to improve the robustness of our framework and correct the expert models when necessary, we fine-tune the router to serve simultaneously as a complementary generator. 
% %
% The router's own logits are trained to provide useful corrective signals on general-domain data, thereby compensating for potential weaknesses of the selected expert models. 
% %
% During inference, we combine the router's logits with those of the chosen expert to produce the final next-token distribution, enabling more robust and accurate generation. 
%
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{9ea6c0b84f801acce268f5dfb8b04884.png}
%     \caption{The router framework
% }
%     \label{fig:2}
% \end{figure}
In summary, we have the following contributions:
\begin{itemize}[leftmargin=*,noitemsep]
    \item We propose \algname, a token-level approach that automatically selects the most suitable expert model at each decoding step while simultaneously providing a complementary logit for better generation.
    
    \item Theoretically, we show that expert-only token-level collaboration as in~\citep{chakraborty2025collab} cannot in general attain the optimal value function unless strong assumptions hold, revealing a fundamental limitation of prior methods. 
    %
    In contrast, \algname's complementary generator overcomes this limitation and enables recovery of the optimal policy.
    %

    \item
    Empirically, \algname consistently outperforms strong baselines---including token-level collaboration methods, model merging, and even finetuned models---across diverse expert domains (mathematics, coding, and instruction following) as well as general-purpose evaluations. 
    %
    These results highlight \algname's robustness, efficiency, and broad applicability in scenarios where expert strengths differ.
    %
    
    % We train a token-level router model that can both be a good model selector and a good complementary generator. The model selection part is trained to output a weight over candidate models given each prefix, and we choose the model with the maximum weight to generate the next one token during inference. This part is trained only on uncertain tokens, which are positions in the expert data where multiple expert models have different predictions on this position. This allows it to focus on the meaningful parts of the expert data and avoid unlearning. Additionally, the router’s base model is trained in a complementary manner so that it can correct the expert models when necessary. 
    % The resulting framework is efficient and flexible to enable collaboration between expert models with different structures, different sizes, and different expertise without jointly training them.
    % \item Theoretically, we first show that our router-based selection strategy can approximately achieve the optimal value by training directly on the expert data, under the assumption that for every possible prefix, there exists at least one expert model that serves as a good approximator of the optimal policy. In contrast, prior controlled-decoding approaches fail to reach this optimal value under the same setting. We then prove that if this assumption holds only for sub-exponential possible prefixes, achieving the optimal value function becomes impossible without enumerating an exponential number of candidate continuations, implying a fundamental limitation for token-level multi-agent collaboration (MAC) methods that rely solely on expert models. Finally, we show that introducing a well-trained complementary generator enables us to recover the optimal value function, overcoming the limitations of expert-only collaboration.
    % \item Empirically, we evaluate our token-level MAC approach on both cross-domain datasets and general datasets. On both datasets, our model achieves the best performance over several baselines, including model merging, controlled-decoding token-level MAC approaches and finetuned models without expert models. 
\end{itemize}

% \textbf{Structure} Section 2 discusses some related works, and Section 3 describes the basic router architecture. Section 4 introduces the router training strategy for both the model selection part and the complementary generating part. Section 5 provides theoretical evidence of the effectiveness of our framework. Section 6 shows all the empirical results for both cross-domain performance and the general GPT4 win rate on general datasets.

% \section{Motivation}

% Recent studies have focused on test-time alignment, bypassing the need for LLM fine-tuning. These approaches utilize controlled decoding with trajectory-level reward functions to align target rewards (ARGS, CARDS). However, they face challenges: either evaluating partial responses with trajectory-level reward functions, which is inaccurate, or generating full responses for next-token prediction, which is inefficient.
% GenARM tackles this issue by employing a token-level reward function, enabling efficient decoding through standard training procedures.
% Despite this, RLHF remains challenging when the base model fails to match the target task. Consequently, single-agent models struggle with diversity and comprehensiveness. To address this limitation, Collab introduces a multi-agent model with controlled decoding, effectively selecting a better reference policy that matches the target task.
% However, the current implementation requires generating full responses multiple times to evaluate the Q function and selecting the best LLM for each token. However, since it needs to generate the full responses for each token during the decoding process, it is super inefficient. Hence, how to fully utilize the advantage of the token-level autoregressive reward model to reduce the computational cost is an important problem. In this project, we aim to train a router that can pre-allocate the models or the weights of different models, and then only chooses these models to generate the next token. If we allocate one model for each token, the computational cost of our decoding process is much more efficient and almost equals to the standard single-agent decoding. If we allocate the weights for several models and merge the logits by the weights, it allows a more flexible decoding process and bring a better performance. 

==> tex/method.tex <==
\section{\algname}
\subsection{Overall Design}
\label{gen_inst}
% \zz{I think the high-level logic/overview is mixed with implementation details too early. I will try re-writing this section. Feel free to edit/merge.}

% \zz{TODO: main figure of \algname}


\algname enables token-level collaboration among specialized LLMs by selecting the most suitable expert at each decoding step while remaining robust to unreliable experts. Pure expert selection is often brittle, as even strong specialists can fail on out-of-domain inputs.
%
\algname addresses this challenge by introducing a router that simultaneously selects the appropriate expert and supplies a complementary logit to refine the expert’s prediction.
%

The \algname router model $\pi_\theta$ is post-trained from a base LLM parameterized by $\theta_{\mathrm{LM}}$. 
%
Given a prompt $x$ and a partial generation $y_{\le t}$, \algname processes the sequence and produces two outputs: a vector of routing weights $w_\theta \in \mathbb{R}^n$, which determines the preferred expert from a set of specialized LLMs $\{\pi_1, \ldots, \pi_n\}$, and a set of logits $\log \pi_{\theta_{\mathrm{LM}}}(\cdot \mid x, y_{\le t})$, which act as a complementary corrective component. 
%
The routing weights are generated via a lightweight linear projection applied to the final hidden state $h_{\theta_{\mathrm{LM}}}(x, y_{\le t})$, namely $\langle W, h_{\theta_{\mathrm{LM}}}(x, y_{\le t})\rangle$. 
%
% Despite its simplicity, this mechanism enables token-level expert assignments that adapt smoothly to the evolving context.
%

During inference, \algname first selects the expert with the highest routing weight, $I^*_\theta = \arg\max_i w_{\theta,i}$, and uses $\pi_{\text{expert}} = \pi_{I^*_\theta}$ as the selected specialist model for the current step. 
%
The final next-token distribution is then obtained by combining the router's \textit{complementary} logits with those of the selected expert through logit addition,
%
\begin{align}
    &\log \pi_{\text{final}}(\cdot \mid x, y_{\le t})
= \log \pi_{\theta_{\mathrm{LM}}}(\cdot \mid x, y_{\le t})
+ \log \pi_{\text{expert}}(\cdot \mid x, y_{\le t}).\label{eq:combine}
\end{align}
%
The next token $y_{t+1}$ is generated from $\pi_{\text{final}}$.
%
This design preserves the domain-specific strengths of the selected expert while allowing the router to correct expert behavior when necessary. 
%
Because the router and routing layer are trained on mixed-domain data, the complementary logits also help anchor generation to distributions observed during training, improving stability and robustness in settings where expert outputs alone are unreliable. 
%
Conceptually, \algname transforms token-level collaboration from a brittle expert-selection problem into a more expressive policy that blends fixed expert knowledge with a learned, adaptive corrective component. 
%
As shown in \secref{sec:theoretical_analysis}, this complementary mechanism is essential for overcoming the fundamental limitations of purely expert-based token-level collaboration.
%


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/5391767045229_.pic.jpg}
    \caption{
    \textit{Top:} Overall architectural design of \algname. 
    %
    \algname enables multiple specialized LLMs to work collaboratively through a carefully designed router. 
    %
    The router outputs \textit{both} the weights for token-level routing and the logits to complement the experts' output. 
    %
    % The output logits are first trained using SFT data.
    %
    \textit{Bottom:} The training process is decomposed into two phases. 
    %
    In the SFT phase (\secref{subsubsec:sft}), the router learns token-wise mixture weights over the expert models and is jointly fine-tuned to become a good response generator.
    %
    In the CDPO phase (\secref{subsubsec:cdpo}), \algname refines the final policy by using preference optimization to improve upon the experts’ outputs.
    %
    }
    \label{fig:fusionRoute}
\end{figure*}

% Suppose we have $n$ LLMs $\{\pi_1,\cdots, \pi_n\}$, initial prompt $x$, and generated tokens $y_{\le t} = y_1\cdots, y_t$ at step $t$, the router's ability is to automatically allocate models for collaboration and generating new token $y_{t+1}$.
% %
% Our router $\pi_{\theta}$ builds upon base language model with parameter $\theta_{\text{LM}}$.
% %
% To enable token-level routing, we augment the model by appending a linear projection layer $\langle W, h_{\theta_{\text{LM}}}(x,y)\rangle $ with parameter $W \in \RR^{n \times d_{\text{hidden}}}$ to its final hidden state $h_{\theta_{\text{LM}}} (x,y) \in \RR^{d_{\text{hidden}}}$, where $d_{\text{hidden}}$ denotes the hidden dimension of the last layer. The final output is an $n$-dimensional vector $w_\theta \in \RR^n$.
% %
% % Hence, the parameter of the router $\theta = (\theta_{\text{LM}}, W)$  
% The router receives the previous tokens $x,y_{\le t} =x, y_1,\cdots, y_t$, and then generate $n$-dimensional weights $w_\theta$ and also the logits $\log \pi_{\theta_{\text{LM}}}(\cdot \mid x,y_{\le t})$. 
% %
% These weights represent the prediction from the router about the candidate model's capability to generate a good next token, and the router's logits act as a complementary part, allowing the router to refine or correct the expert's outputs rather than relying solely on the candidate models.
%

% During inference, at time $t$, we first choose the model $\pi_{\text{expert}} = \pi_{I^*}$ where $I^*_\theta=\arg \max_{i \in [n]} ( w_i)$ maximize the weight. Then, we aggregate the logits as \begin{equation}\log \pi_{final}(\cdot \mid x,y_{\le t}) = \log \pi_{\theta_{\text{LM}}}(\cdot \mid x,y_{\le t}) + \log \pi_{\text{expert}}(\cdot \mid x,y_{\le t})\label{eq:combine}\end{equation} and  generate the next token $y_{t+1} = \arg\max_{y \in \mathcal{Y}}\log \pi_{final}(y_{t+1} \mid x,y_{\le t})$ using greedy decoding. 
% % \hz{For option 1 under E2E training (5.1.4), is it following the standard sparse top-K gate training in MoE, like \url{https://arxiv.org/abs/1701.06538} or \url{https://arxiv.org/pdf/2101.03961} (except that we don't have load-balance loss)?}
%  While relying only on the selected candidate model $\pi_{I^*}$ provides domain-specific knowledge, it may still yield low-quality responses in ambiguous or out-of-distribution cases. Therefore, the router model $\pi_{\theta}$ must play a dual role: guiding candidate model selection and providing a complementary component that improves the robustness of the final output. This collaboration stabilizes the decoding process and enhances the overall quality of the generated text. Moreover, since the routing part and router base model are trained on the same training dataset, incorporating the router's logits $\log \pi_\theta$ during decoding can help the generation process align with the data distribution seen during training, hence improving consistency and reinforcing the effectiveness of the routing.
% % Another approach let the candidate model generate the next token, and then choose one with largest router logits within these topk models, i.e., $i^* = \arg\max_{i \in I^*} z_{r,t}(y_{i,t+1})$, where $y_{i,t+1}$ is the next token generated by model $i$, and $z_{r,t}(y)$ for some token $y$ means the logit of this token. 
% % \hz{For option 2, wondering how would we do the training, as $\arg\max$ is non-differentiable?}
% % The details are provided in Section \ref{sec:approach}

% Our goal is to align the human preference. To evaluate the next token generation, we can learn a token-wise reward function like GenARM. The goal is to maximize the overall target reward. 





% \section{Approach}
% \label{sec:approach}


% \subsection{Multi-Agent Collaboration with GenARM (GenARM MAC)}

% The trivial algorithm without router is to use autoregressive token-level reward model to evaluate the quality of several next tokens generated by $n$ models. At each timestep $t$, assuming that we have generated $y_{\le t},$ then for each LLM $M_i, i \in [n]$, we generate $k$ candidate tokens $c_1^{(i)}, \cdots, c_k^{(i)}=\mathrm{topk}(M_i(x,y_{\le t}))$ with logits $z_1^{(i)}, \cdots, z_k^{(i)}$. Then, we compute the logits of the auto-regressive token-level reward model $z_{1,r}^{(i)}, \cdots, z_{k,r}^{(i)}$. The final score of the model $M_i$ will be finally defined by 
% $$s_i = \max_{j\in [k]}(z_j^{(i)} + z_{j,r}^{(i)}),$$
% and the selected token will be $c^{(i)}=c_{s_i}^{(i)}$.

% Now, after the score calculation, we finally choose the model with highest score, i.e., $i^* = \arg\max_i s_i,$ and we choose the next token $y_{t+1}=c^{(i^*)}$. In fact, this approach can be regarded as applying auto-regressive token-level reward model to evaluate the quality of the next token, and use it for model selection and collaboration. 

% \subsubsection{Router for Model Selection}

% Our second approach is called Router for Model Selection (RMS). At timestep $t$, we first called the router to get $f(x,y_{\le t})=w_1,\cdots, w_n$. Hence, we choose $i^\dagger = \arg\max_{i \in [n]} w_i$ as the next model. Now we compute $k$ candidate tokens $c_1,\cdots, c_k$ and the logits of them $z_1,\cdots, z_k$ by model $M_{i^{\dagger}}$. After that, we compute the logits of the auto-regressive reward model as $z_1^r,\cdots, z_k^r$, and we choose the next token as $y_{t+1}=c_{i^*},$ where $i^* = \arg\max_{i \in [k]}(z_i^r + z_i)$. The computational cost of this algorithm is significantly less than the GenARM MAC since we do not need to execute decoding for each LLM at each token. When the number of models are large, it will be significantly smaller.

% \subsection{Router for Model Combination}

% Our next approach is called Router for Model Combination (RMC). At timestep $t$, we also called the router to get $f(x,y_{\le t})=w_1,\cdots, w_n$. Without loss of generality, we assume $w_1>w_2>\cdots>w_n$. Instead of choosing one particular model with the highest weight, we take $p$ models $M_1,\cdots, M_p$ with top-$p$-weight. We then perform softmax transformation to get the new weight $\{w_i'\}_{1\le i\le p}= \mathrm{Softmax}(\{w_i\}_{1\le i\le p}).$

% Now we first combine $p$ logits of different models as  $z=\sum_{i \in [p]} w_i'z_i$, where $z_i$ is the logits of the model $M_i$. Then, we compute $k$ candidate tokens $c_1,\cdots, c_k$ by choosing top-k tokens $z^{(1)}, \cdots, z^{(k)}$ by logits $z$. After that, we calculate the logits of the auto-regressive reward model for these $k$ tokens as $z^{(1),r},\cdots, z^{(k),r}.$ We now combine the logits and choose the tokens with largest logits by $y_{t+1}=c_{i^*}$, where  $i^* = \arg\max_i (z^{(i)} + z^{(i),r})$.

% The computational cost of this approach highly depends on the selection of $p$. When $p=1$, this algorithm is equivalent to the RMS. When $p=n$, this algorithm has a similar computational cost to the GenARM MAC. However, this approach allows a more flexible collaboration in the token-logit-level. 

\subsection{Training \algname}
% \zz{Imo the goal of each phase is not explicit enough.}


Having introduced the routing-and-complementation framework of \algname, we now describe how the router is trained. Training \algname is non-trivial since the router must \textit{simultaneously} satisfy two coupled objectives: 1) it must reliably select the most suitable expert at each token, while 2) also providing a complementary logit contribution that corrects expert failures when necessary. 
%
Naively optimizing these objectives together can lead to unstable behavior, where improvements in complementary generation degrade routing quality or vice versa. 
%
To address this challenge, we adopt a staged and decoupled training strategy consisting of supervised fine-tuning (SFT) followed by a modified preference-optimization phase.
%

% In this section, we introduce the training methodology for our router, covering both the model-selection component and the complementary component. We begin with SFT, which equips the router with basic generation capability while simultaneously learning to select the appropriate expert model. To further strengthen the router’s ability to complement the candidate model and improve overall performance, we use a modified version of DPO to help the router learn complementary parts of the candidate models, enabling it to improve the quality of the final generated responses.
% \label{sec:router training}
% % \subsection{Training Data}
% \subsection{Labeling}
% \subsubsection{Expert Label}
% One approach to train the router is to assign the labels for model index for the text. 
% Hence, we need to first compute the score labels for the router. For a pre-collected dataset, for each sentence $(x,y)$ and each token, we compute the score for all LLMs. To be more specific, we compute the logits  for $y_{t+1}$ using  LLM $M_i$ given $(x,y_{\le t})$. Denote them to be $\{z^{(i)}\}_{i \in [n]}$. Then for the LLM $M_i$, its score is defined by the logits of $z^{(i)}$ from an expert model (usually a bigger model like fine-tuned Llama 30B). Finally, we construct hard labels by uniformly distributing probability mass over all indices that share the maximum score in the vector. 
% \subsubsection{SFT label}
% We also try construct hard labels using logits of all models. For the text $(x,y)$, the score of model $M_i$ token $y_{t+1}$ is defined by the logits of $y_{t+1}$ from the model $M_i$, and then we choose the hard label with maximum score as the training labels.
% \subsubsection{Mixed Label}

% Since we utilize models with different areas of expertise, we can mix diverse datasets—such as math, code, and instruction-following—to train the expertise. The labels are determined by the source of each training sample. For instance, for data originating from the math dataset, all tokens are labeled to indicate that the router should select the math expert model.

\subsubsection{Supervised fine-tuning (SFT)}\label{subsubsec:sft}

We first perform SFT to establish two foundational properties of the router: next-token prediction capability and token-level expert selection. 
%
Importantly, this phase is not intended to train the router's complementary behavior, but rather to produce a stable routing mechanism aligned with expert specialization.
%
During SFT, we jointly optimize the base LLM parameters $\theta_{\text{LM}}$ and the routing projection $W$ using a combination of a standard language modeling loss and a routing loss.
%
The language modeling loss $\mathcal{L}_{\text{LM}}(\theta_{\text{LM}};x,y)$ given the data point $(x,y)$ follows the standard SFT objective and encourages accurate next-token prediction on the training data. 
 %\yh{we can put this sentence at the end of the whole subsection?}
 
To enable token-level routing, we introduce a routing loss that favors experts whose predictions align with the ground-truth sequence. 
%
However, many tokens (e.g., punctuation or function words) provide little routing signal because all experts predict them similarly. 
%
Supervising on such tokens can dominate the gradient and bias the router toward uninformative agreement. We therefore restrict routing supervision to token positions where experts disagree.
%

For a given prefix $(x, y_{\le t})$, let
$y_{i,t+1} = \arg\max_y \log \pi_i(y \mid x, y_{\le t})$ denote the next-token prediction of expert $\pi_i$. 
%
We define the \textit{informative} token set as
%
$
    \mathcal{S} = \{ t \in [T] : \exists i \neq i' \text{ such that } y_{i,t+1} \neq y_{i',t+1} \}.
$
%
For these positions, at token $t$, we first compute the router weight $w_{\theta}^t$ and compute the aggregated logits as
%
\begin{equation}
   \log \pi_{\text{agg}}(\cdot \mid x,y_{\le t}) = \sum_{i=1}^n w_{\theta, i}^t \log \pi_{i}(\cdot \mid x, y_{\le t}), 
\end{equation}
%
where the weight $w_{\theta}^t = (w_{\theta,1}^t, \cdots, w_{\theta,n}^t)$ represents the output of the linear layer for token $t$ under parameter $\theta$, and define the routing loss
as
$
    \cL_{\text{expert}}(\theta;x,y) = \sum_{i \in S}-\log \pi_{\text{agg}}(y_i \mid x,y_{\le i-1}).
$
%
% Let $y_{i,t+1}=\arg \max_{y \in \mathcal{Y}} \log \pi_i(\cdot \mid x,y_{\le t})$ denote the decoding result for the model $i$ at step $t$. 
%
% For each prompt-response pairs in the SFT data $(x,y_{\le T}) \in \cD_{\text{SFT}}$, we identify the set of token positions where different experts produce different predictions: $S = \{t \in [T]:  \exists i,i' \in [n], y_{i,t}\neq y_{i',t}\}$.
%
The final SFT objective therefore is
%
\begin{equation}\label{eq:sftloss}
\cL_{\text{SFT}}(\theta)=\EE_{(x,y) \in \cD_{\text{SFT}}}\left[\cL_{\text{LM}}(\theta_{\text{LM}};x,y) + \lambda\cL_{\text{expert}}(\theta;x,y)\right],
\end{equation} 
%
where $\lambda$ is some hyperparameter for balancing the scale of two losses.
%
By restricting supervision to informative tokens, this objective ensures that routing gradients are driven by meaningful expert disagreements, allowing the router to capture expert specialization without being dominated by trivial agreement cases.
%
% This token selection strategy prevents the router from unlearning by avoiding supervision on tokens where all experts agree.

% Without this filtering, the router would receive strong gradients
% \hz{Curious why the ``consistent'' tokens will generate strong gradients? Tokens outside S will have similar $\log \pi_i(\cdot | x, y_{\leq t})\approx \log \pi'$. Then $\log\pi_\text{agg} = (\sum w)\cdot \log \pi' = \log \pi'$. So gradient on $w$ is close to 0?} from a large number of trivial tokens (e.g., punctuation or common words), which convey little information about model specialization.
% As a result, it could overfit to these non-informative tokens and fail to capture meaningful routing behavior. Note that in this SFT phase, we only train the router to give it basic generation ability, instead of training it as a complementary part.

%\hz{if we already have ground-truth next token, what's the benefit of explicitly constructing labels of expert indices? Intuitively, E2E training should be better?}

% \textbf{DPO}
\subsubsection{Complemented Direct Preference Optimization (CDPO)}\label{subsubsec:cdpo}
% While SFT provides the router with basic generative ability, it does not sufficiently teach the router when and how to provide complementary signals beyond the selected expert. 
While SFT establishes routing and preserves next-token prediction, it does not address how the router should correct locally suboptimal expert outputs. In practice, experts may produce unreliable logits even when correctly selected. We therefore introduce a preference optimization phase that trains the router to learn complementary logit contributions while treating expert outputs as fixed.
%
We refer to this preference-optimization stage as Complemented Direct Preference Optimization (CDPO).

% Training such a router model without influencing the established routing ability is non-trivial. 
% %
% Our router must preserve its ability to dynamically select the expert models, while simultaneously improving its complementary ability and the quality of the final output once the expert outputs are integrated.
% To address these challenges, our training procedure introduces two key modifications to the classical DPO framework.

% \textbf{Complement Training} 
During inference, the final policy is obtained by combining the router and the selected expert model logits through logits addition, as shown in \eqnref{eq:combine}.
%
To align training with this decoding behavior, we introduce a \textit{preference-optimization objective} that applies Direct Preference Optimization (DPO)~\citep{rafailov2023direct} to the router's base model parameters $\theta_{\mathrm{LM}}$. 
%
% Given preference pairs $(x, y^{w}, y^{l})$ for the same prompt $x$, the objective is defined as
% \begin{small}
% \begin{align}
% &\mathcal{L}_{\text{CDPO}}(\theta_{\text{LM}})\nonumber\\
% & = -\mathbb{E}_{x, y_w, y_l \in \mathcal{D}_{\text{DPO}}}
% \Bigg[
% \log \sigma \Bigg(
% \sum_{t \ge 0}
% \beta \log 
% \frac{
% \pi_{\text{final}}(y_{t+1} \mid y_{w,\le t}, x)
% }{
% \pi_{\text{ref}}(y_{t+1} \mid y_{w,\le t}, x)
% }
% -
% \sum_{t \ge 0}
% \beta \log 
% \frac{
% \pi_{\text{final}}(y_{t+1} \mid y_{l,\le t}, x)
% }{
% \pi_{\text{ref}}(y_{t+1} \mid y_{l,\le t}, x)
% }
% \Bigg)
% \Bigg]\nonumber\\
% &= -\mathbb{E}_{x, y_w, y_l \in \mathcal{D}_{\text{DPO}}}
% \Bigg[
% \log \sigma \Bigg(\Big(\underbrace{
% \sum_{t \ge 0}
% \beta \log 
% \frac{
% \pi_{\theta_{\text{LM}}}(y_{t+1} \mid y_{w,\le t}, x)
% }{
% \pi_{\text{ref}}(y_{t+1} \mid y_{w,\le t}, x)
% }
% -
% \sum_{t \ge 0}
% \beta \log 
% \frac{
% \pi_{\theta_{\text{LM}}}(y_{t+1} \mid y_{l,\le t}, x)
% }{
% \pi_{\text{ref}}(y_{t+1} \mid y_{l,\le t}, x)
% }}_{\text{(A)}}
% \Big)\nonumber\\ 
% & \qquad + \Big(\underbrace{\sum_{t \ge 0}
% \beta \log 
% \frac{\pi_{\text{expert}}(y_{t+1} \mid y_{w,\le t}, x)}{\pi_{\text{expert}}(y_{t+1} \mid y_{l,\le t}, x)}
% }_{\text{(B)}}\Big)\Bigg)
% \Bigg],\label{eq:cdpo_loss}
% \end{align}
% \end{small}
% %

Given preference pairs $(x,y^{w},y^{l})$ for the same prompt $x$, for any policy $\pi$, define the contrastive loss as 
\begin{align*}
r_{\pi}(x,y, y_l)
:=
\sum_{t\ge 0}\beta\log
\frac{\pi(y_{t+1}\mid y_{w,\le t},x)}{\pi_{\rm ref}(y_{t+1}\mid y_{w,\le t},x)} - \sum_{t\ge 0}\beta\log
\frac{\pi(y_{t+1}\mid y_{l,\le t},x)}{\pi_{\rm ref}(y_{t+1}\mid y_{l,\le t},x)}  .
\end{align*}
The objective is defined by 

\begin{align}
\mathcal{L}_{\rm CDPO}(\theta_{\rm LM})&= -\mathbb{E}_{(x,y_{w},y_{l})\sim\mathcal{D}_{\rm DPO}}
\Big[\log \sigma\Big(\ell_{\pi_{\text{final}}} (x,y_w, y_l)\Big)\Big]\nonumber\\&=-\mathbb{E}_{(x,y_{w},y_{l})\sim\mathcal{D}_{\rm DPO}}
\Big[\log \sigma\Bigg(\ell_{\pi_{\theta_{\text{LM}}}} (x,y_w, y_l) +\underbrace{\sum_{t \ge 0}
\beta \log 
\frac{\pi_{\text{expert}}(y_{t+1} \mid y_{w,\le t}, x)}{\pi_{\text{expert}}(y_{t+1} \mid y_{l,\le t}, x)}
}_{\text{(Bias)}}\Bigg)
\Bigg],
\label{eq:cdpo_loss}
\end{align}
where $\pi_{\text{ref}}$ denotes the router after the SFT phase, $\sigma(x) = (1+e^{-x})^{-1}$ is the sigmoid function, and $\beta$ controls the strength of preference alignment.
%

Importantly, we do not backward propagate any gradient for bias term, hence it can be regarded as an extra token-level bias.
%
Optimizing this loss naturally encourages the router to provide a complementary logit contribution that compensates for the weaknesses in the expert models. 
%
For example, if the expert $\pi_{\text{expert}}$ already provides a strong policy for a given prompt $x$, the log-ratio gap contributed by the expert term is already large, resulting in a small gradient with respect to $\theta_{\text{LM}}$. 
%
Conversely, when $\pi_{\text{expert}}$ is weak for prompt $x$, the log-ratio gap shrinks, producing a larger gradient on $\theta_{\text{LM}}$ that encourages the router to provide stronger corrective logits. 
%
As a result, the router refines expert predictions precisely when needed, improving robustness while aligning training with the collaborative decoding behavior used at inference time.
% As a result, the router learns to be both an expert selector and a complementary next-token generator, improving robustness and aligning training with the collaborative decoding behavior.
%
% \hz{As a reader, I'd be curious: 1. why don't we let complementary logits in SFT (doable by adding to $\log \pi_\text{agg}$), and 2. does it make sense to set $\pi_\text{ref}$ as $\pi_\text{expert}$? Then we are just optimizing $\log\pi_{\theta_{\text{LM}}}$ -- i.e., the complementary part without constraint. Does it also make sense (since it's just complementary)? }\nuoya{ The reason we do not use complementary logits during the SFT phase is that this phase is intended to give the router a basic ability to generate coherent outputs. Introducing complementary logits would be somewhat unnatural, since the cross-entropy loss is defined between the model’s logits and a one-hot label, and combining logits from multiple experts does not align well with this formulation.

% The $\pi_{\text{expert}}$ is the combination of several candidate experts, which is not the $\pi_{\text{ref}}$? In this phase, we instead use $\pi_{\text{ref}}$ as the output in the SFT phase.}
\begin{algorithm}[!t]
     \begin{algorithmic}[1]
         \caption{Mix Training}
         \label{alg:mixdpo}
         %\STATE \textbf{Initial}: Dataset $\cD_i.$
         \STATE \textbf{Initial}: Dataset $\cD_{\text{SFT}}$, $\cD_{\text{DPO}}$, SFT router $\pi_{\theta}$, batch size $B$, learning rate $\eta$.
         \STATE Mix two datasets randomly to get $\cD_{\text{mix}}$.
         \FOR{$t=1,2,\cdots,$}
            \STATE Receive a batch of data points $\{d_1,\cdots, d_B\}\in \cD_{\text{mix}}$. Set $\cL = 0.$
            \FOR{$i=1,2,\cdots, B$}
            \IF{$d_i = (x,y) \in \cD_{\text{SFT}}$}\STATE $\cL = \cL + \lambda \cL_{\text{expert}}(\theta; d_i)$.
            \ELSE
                \STATE $\cL = \cL + \cL_{\text{CDPO}}(\theta_{\text{LM}}; d_i)$.
            \ENDIF
            \ENDFOR
            \STATE Update the parameter $\theta = \theta - \eta \nabla_\theta \cL.$
         \ENDFOR
     \end{algorithmic}
\end{algorithm}

\subsubsection{Mix Training}
Since preference optimization updates the router's base model parameters $\theta_{\text{LM}}$, it can indirectly influence the routing behavior through shared representations. 
%
% It is therefore necessary to maintain both routing and complementary capabilities during training. 
It is therefore necessary to preserve both reliable expert selection and effective complementary logit refinement during training.
%
A naive approach would be to apply the DPO objective directly to the entire router, including its final linear routing layer. 
%
However, doing so often leads to unstable or degenerate routing behavior, where the linear routing layer overfits to preference-alignment signals and loses its ability to correctly select among experts. 
%

To address this issue, we adopt a decoupled optimization strategy.
%
Specifically, for SFT samples, all parameters, including the routing layer, are updated using the routing loss $
\mathcal{L}_{\mathrm{expert}}$. 
%
On the other hand, we apply the preference-optimization objective (\eqnref{eq:cdpo_loss}) only to the router's base model parameters $\theta_{\text{LM}}$, while excluding the routing projection.
%
To ensure consistency between the base model and the linear layer, we jointly mix preference-optimization data with supervised SFT data during training. 
%
% All parameters $\theta$ including linear layer are also updated by minimizing the routing loss $\lambda \mathcal{L}_{\text{router}}$ computed on the SFT dataset, while the base model parameters continue to be optimized with the DPO objective.
%
This mixed training scheme preserves expert-selection capability while enabling the router to acquire an effective complementary logit contribution.
%
The full procedure is summarized in Algorithm~\ref{alg:mixdpo}.
% This joint training scheme makes the router a good complementary generator without reducing its model-selection capability. 
%
% The pseudocode is shown in Algorithm~\ref{alg:mixdpo}.
%



% \subsection{Router Structure}

% Our router is fine-tuned from a base language model (Llama3.1-8B), with variations depending on the experimental setup. To enable token-level routing, we augment the model by appending a linear projection layer to its final hidden state, producing an $n$-dimensional output vector. The training objective combines two components: a language modeling loss and a score loss. The score loss is computed using BCE loss between the predicted scores and the target scores provided by a larger expert model. The language modeling loss follows the standard SFT objective, encouraging the model to generate the next token in the target sequence.

==> tex/preliminary.tex <==
\section{Preliminaries}
\subsection{LLM Decoding}
We formalize the decoding process of a language model as sampling from an autoregressive policy $\pi$. Let $\mathcal{X}$ denote the space of prompts and $\mathcal{Y}$ the vocabulary. A response is represented as a sequence $y=(y_1,\dots,y_T)\in\mathcal{Y}^T$.
Given a prompt $x\in\mathcal{X}$, the language model induces a conditional distribution over responses through the policy
\[
\pi(y\mid x)=\prod_{t=1}^T \pi(y_t\mid x, y_{<t}),
\]
where $\pi(y_t\mid x, y_{<t})$ specifies the probability of generating token $y_t$ given the prompt and the preceding tokens.
In both the empirical part and the theoretical part of our paper, we consider the greedy decoding, since it is the simplest and effective way for decoding. To be more specific, at each step $t$ greedy decoding selects the token with the highest conditional probability under the policy $\pi$:
$
y_t = \arg\max_{y \in \mathcal{Y}} \pi(y \mid x, y_{<t}).
$
\subsection{SFT and RLHF}
Supervised fine-tuning (SFT) initializes the language model by training it to imitate human-written demonstrations via supervised learning, enabling the model to acquire basic capabilities and generate high-quality responses. Building on the resulting model $\pi_{\text{ref}}$, a widely used RLHF method is DPO \citep{rafailov2023direct}, which aligns the model with human preferences using annotated preference pairs. Given $(x, y^+, y^-)$, where $y^+$ and $y^-$ denote the preferred and dispreferred responses, DPO derives a closed-form objective from the Bradley–Terry model, enabling policy updates through a purely supervised loss.

\begin{equation*}
\mathcal{L}_{\text{DPO}}(\theta) = 
-\log \sigma\left(
\beta \left[
\frac{\log \pi_\theta(y^+|x)}{\log \pi_{\text{ref}}(y^+|x) } - \frac{\log \pi_\theta(y^-|x)}{\log \pi_{\text{ref}}(y^-|x)}
\right]
\right),
\end{equation*}
where $\beta$ controls the strength of alignment. 

% We further assume a reward function $r:\mathcal{X}\times\mathcal{Y}^T\to\mathbb{R}$ that evaluates the quality of a generated response given its prompt. This formulation provides a formal basis for analyzing and optimizing LLM decoding behaviors under arbitrary reward functions.

% We formulate the decoding process as a token-level Markov Decision Process (MDP) $\cM = \{\cS, \cA, \PP, r\}$, where $\cS$ is the state space, $\cA$ is the action space, $\PP$ is the transition kernel, and $r$ defines the reward function. 
% %
% In the language model setting, let the prompt space be $\cX$ and the vocabulary be $\cY$.
% %
% Starting from an initial prompt $s_0=x$, at step $t$ the state is defined by $s_t = (x, y_{\le t}),$ and the action is represented by the next token $a_t = y_{t+1}$. 
% %
% The transition kernel is then defined by $\PP(s_{t+1}\mid s_t, a_t) = \II\{s_{t+1}=(x, y_{\leq t}, y_{t+1})\}$.
% % \hz{$(x, y_{\leq t}, y_{t+1})$?}. 
% %
% Finally, the reward function $r(s,a) = r(x,y_{\le t+1}) \in \RR$ is a token-level reward function that maps any text $(x,y_{\le t+1})$ to a real number.
% %

% A language model can be represented as a policy $\pi(a\mid s) = \pi(y_{t+1} \mid x,y_{\le t})$, where it takes the previous text $(x,y_{\leq t})$ as the input and generates the next token $y_{t+1}$.
% %
% Let $\tau = (x,y_{1}, \cdots, y_T)$ denote the trajectory, which is indeed a full response generated by a language model, the value function $V^\pi(s) = V^\pi(x,y_{\le t})$ for a state $s = (x,y_{\le t})$ can be defined as
% %
% \begin{align*}
%     V^\pi(x, y_{\le t}) =\EE_{\tau \sim \pi(\cdot \mid x,y_{\le t})}\left[\sum_{i=t+1}^{T} r(x, y_{\le i}) \right].
% \end{align*}
% %
% Similarly, for $a = y_{t+1}$, the Q function can be defined as
% %
% \begin{align*}
%     Q^\pi(x, y_{\le t}, y_{t+1})  = r(y_{t+1};x, y_{\le t}) + \EE_{\tau \sim \pi(\cdot \mid x,y_{\le t+1})}\left[\sum_{i=t+1}^T r(y_{i+1};x, y_{\le i})\right].
% \end{align*}
% %

==> tex/related_work.tex <==
\section{Related Works}
\subsection{Multi-LLM Collaboration}
Recent advances in LLMs have shown that sufficiently large, general-purpose LLMs can achieve strong performance across a wide range of tasks, including mathematics, coding, and instruction following~\citep{hurst2024gpt, team2025gemma, yang2025qwen3, zeng2025glm}.
%
However, such models are often prohibitively expensive to train and deploy, motivating interest in more efficient alternatives.
%
At the same time, smaller and domain-specialized LLMs can perform competitively within their respective domains, but typically struggle to generalize beyond the distributions on which they are trained.
%
Bridging this gap between specialization and generalization without incurring the cost of training ever-larger models has therefore become an important challenge.
%
% In recent years, because of the existence of diverse downstream tasks, a single LLM is hard to perform well in diverse downstream tasks such as math, coding, instruct-following and chat generation. 
%
% Motivated by the fact that different models may have different capabilities and advantages, many works consider how to incorporate multiple LLMs to generate a better response compared to a single LLM and perform better on a diverse dataset. 
%
One line of works study the benefits of multi-agent debate, in which several agents discuss and debate to generate a final response~\citep{liu2024groupdebate, chan2023chateval, liang2024encouraging}. 
%
Existing works also try to model the social and economic behavior in the real world using different specialized LLMs~\citep{zhao2023competeai}.
%
Moreover, model ensemble methods~\citep{ashiga2025ensemble,huang2024ensemble,chen2025harnessing} combine responses or probability distributions from multiple models in a fixed manner to leverage their complementary strengths without modifying individual parameters; however, they lack dynamic, context-dependent collaboration among candidate models.
%
More fine-grained token-level collaboration has been studied in recent years. 
%
Collab~\citep{chakraborty2025collab} uses a controlled decoding-based approach to evaluate the candidate tokens during decoding. 
%
Compared to them, our decoding algorithm is much more efficient and also achieves a better performance. 
%
Some papers \citep{shen2024learning, fu2025r2r} also explores token-level collaboration, but mainly uses one strong expert to assist a small fine-tuned model, and its output depends entirely on the candidate experts. 
%
In contrast, we use multiple specialized LLMs, evaluate both cross-domain performance and general win rate, and additionally train the router as a complementary generator to improve robustness.
%

\subsection{Multi-LLM Integration} 
Beyond multi-agent LLM collaboration, a substantial body of works also consider how to utilize and integrate different models to be comprehensive. 
%
The most representative area is Mixture-of-Expert (MoE), in which multiple expert models are combined for each layer with some routing network, allowing the system to leverage the specialized knowledge of each expert for different inputs~\citep{zhou2022mixture, xue2024openmoe, jiang2024mixtral}. 
%
However, because the final architecture tightly integrates the layers of multiple models with a routing network, these approaches are typically applicable only to models with similar structures. 
%
They also require access to the experts' gradients and joint training of the entire system, which limits flexibility and incurs significant additional training cost. 
%
Model merging is another approach for integrating multiple experts~\citep{yu2024language, ilharco2022editing, yadav2023ties}. 
%
While it does not incur additional training costs, its performance is often limited and sensitive to hyperparameters. 
%
Moreover, its flexibility is also limited, as it requires all models to share the same architecture. 
%
There is also a line of work on pluralistic alignment, in which multiple models with potentially conflicting objectives, such as safety and helpfulness, are integrated to achieve tradeoffs across multiple objectives~\citep{shi2024decoding, xiong2025projection, wang2025mpo}.
%
In contrast to these approaches, \algname does not merge or jointly train expert models, nor does it require architectural compatibility or gradient access.
%
Instead, \algname enables flexible, token-level integration of heterogeneous, off-the-shelf LLMs by learning a lightweight router that selects among experts and provides complementary logits during decoding.
%
This design allows \algname to combine the strengths of specialized models while retaining robustness and generalization, without the rigidity or training overhead inherent in MoE and model-merging approaches.
%


==> tex/theory.tex <==
\section{Theoretical Analysis}\label{sec:theoretical_analysis}
\subsection{Token-level Markov Decision Process}\label{subsec:token_level_mdp}
We formulate the decoding process as a token-level Markov Decision Process (MDP) $\cM = \{\cS, \cA, \PP, r\}$, where $\cS$ is the state space, $\cA$ is the action space, $\PP$ is the transition kernel, and $r$ defines the reward function. 
%
In the language model setting, let the prompt space be $\cX$ and the vocabulary be $\cY$.
%
Starting from an initial prompt $s_0=x$, at step $t$ the state is defined by $s_t = (x, y_{\le t}),$ and the action is represented by the next token $a_t = y_{t+1}$. 
%
The transition kernel is then defined by $\PP(s_{t+1}\mid s_t, a_t) = \II\{s_{t+1}=(x, y_{\leq t+1})\}$.
% \hz{$(x, y_{\leq t}, y_{t+1})$?}. 
%
Finally, the reward function $r(s,a) = r(x,y_{\le t+1}) \in [0,1]$ is a token-level reward function that maps any text $(x,y_{\le t+1})$ to a real number. We also denote $R(x,y_{\le t})=\sum_{i=1}^t r(x,y_{\le i})$ is the total reward function of the prefix $(x,y_{\le t})$. 
%

A language model can be represented as a policy $\pi(a\mid s) = \pi(y_{t+1} \mid x,y_{\le t})$, where it takes the previous text $(x,y_{\leq t})$ as the input and generates the next token $y_{t+1}$.
%
Let $\tau = (x,y_{1}, \cdots, y_T)$ denote the trajectory, which is indeed a full response generated by a language model, the value function $V^\pi(s) = V^\pi(x,y_{\le t})$ for a state $s = (x,y_{\le t})$ can be defined as
%
\begin{align*}
    V^\pi(x, y_{\le t}) =\EE_{\tau \sim \pi(\cdot \mid x,y_{\le t})}\left[\sum_{i=t+1}^{T} r(x, y_{\le i}) \right].
\end{align*}
%
Similarly, for $a = y_{t+1}$, the Q function can be defined as
%
\begin{align*}
    Q^\pi(x, y_{\le t}, y_{t+1}) = r(x, y_{\le t+1}) + \EE_{\tau \sim \pi(\cdot \mid x,y_{\le t+1})}\left[\sum_{i=t+1}^T r(x, y_{\le i+1})\right].
\end{align*}
%


\subsection{Token-Level Routing through the Lens of Performance Difference Lemma}
In this section, we establish a conceptual connection between the Performance Difference Lemma (PDL)~\citep{kakade2002approximately} and our token-level routing training , clarifying how supervised routing can be interpreted through the lens of value-function approximation in a token-level MDP.
%
At a high level, PDL characterizes how deviations from the optimal policy at individual decision steps accumulate into a global performance gap. 
%
\begin{lemma}[Performance Difference Lemma~\citep{kakade2002approximately}]\label{lemma: pdl}
    Denote $\rho \in \Delta(\cX)$ as a distribution over the prompt space. 
    %
    Suppose each response $y$ has length $T$. 
    %
    Then, for any two policies $\pi, \pi^*$, we have
    \begin{align*}
    \EE_{x\sim \rho}\Big[V^{\pi^*}(x) - V^{\pi}(x)\Big] = \sum_{t=0}^{T-1} \EE_{x\sim \rho , y_{\le t} \sim \pi} \Big[V^*(x,y_t) -\EE_{y_{t+1}\sim \pi(\cdot \mid x,y_{\le t})}[Q^*(x,y_{\le t+1})]\Big].
    \end{align*}
\end{lemma}
%
When applied to language model decoding, which is viewed as a token-level MDP as shown in \secref{subsec:token_level_mdp}, this lemma suggests that if, at each token position, the routing mechanism selects an expert whose next-token distribution approximately maximizes the optimal action-value function, then the resulting sequence-level policy will be near-optimal.
%
Our routing loss in the SFT phase can be viewed as an imitation-based approximation of this idealized per-token selection rule, trained on trajectories generated by an optimal (or near-optimal) policy.
%

% \zz{
To formalize this connection, we analyze an idealized setting in which
% } 
the SFT dataset is generated by the optimal policy $\pi^*(\cdot \mid s)$, where $\pi^*$ achieves the optimal value function in the token-level MDP $\cM = (\cS, \cA, \PP, r)$. 
%
% We regard the token-level collaboration as an RL process. The state at step $h$ is $s_h = x, y_{\le h}$ and the action $a \in [M]$ represents the selection of the models, where $M$ is the number of the candidate models. Then, the state transits to $s_{h+1}=[x,y_{\le h+1}]$, where $y_{h+1}\sim \pi_{a}(\cdot \mid x,y_{\le t})$.
% Hence, the optimal token for step $h$ is $y_{t+1}=\arg \max_{\pi^*}[Q^{\pi^*}(x,y_{\le t+1})]$.  We also call the $Q^{\pi^*}$ as the optimal Q-function.
% \zz{
Hence, the optimal next token at step $t$ is given by $y_{t+1} \in \arg\max_{a \in \mathcal{Y}} Q_{\pi^*}(x, y_{\le t}, a)$, and we refer to $Q_{\pi^*}$ as the optimal Q-function.
% }
%
% Here, the Q-function is defined by 
% \begin{align*}
%     Q_h^{\pi^*}(x,y_{\le t+1}) = \mathbb{E}_{\pi^*}\left[\sum_{t'=t}^{H}r(x,y_{\le t'+1})\mid x,y_{t+1}\right].
% \end{align*}
% Hence, , the ideal action is to choose $a_t \in \{1,2,\cdots, n\}$ such that $$i_t = \arg\max_{i \in [n]}\mathbb{E}_{y_{t+1}\sim \pi_{i}(\cdot \mid x,y_{\le t})}[Q^{\pi^*}(x,y_{\le t+1})].$$ 
%
% \zz{Made slight edits since SFT does not observe the optimal policy, only the trajectories.}
Since we trained on the SFT dataset which follows trajectories generated by $\pi^*$, at step $t$ with prefix $(x,y_{\le t})$, the router 
% will learn to mimic 
% \zz{
can be viewed as approximating an expert action that aligns with
% }
the action 
% \zz{
preferred by $\pi^*$
% }
, i.e., the action that maximizes the optimal Q-function 
% \zz{
along the observed trajectory.
% }
%
% Hence, we can derive the total gap between the optimal policy and our router-training approach. Compared to the sentence-level approach, we can achieve a smaller distance between the optimal reward and our derived reward. 
We assume that the router is well-trained so that the expert model chooses the correct model for each prefix, namely, 
\begin{align}
    \label{eq: model selection}
    \pi_{\text{expert}}(\cdot \mid x,y_{\le t})=\pi_I(\cdot \mid x, y_{\le t}),
    % ~~\text{where}~~I=\arg\max_i \EE_{y_{t+1}\sim \pi_i(\cdot \mid x,y_{\le t})}
    % [Q_{\pi^*}(x, y_{\le t}, y_{t+1})].
\end{align}
where $I=\arg\max_i \EE_{y_{t+1}\sim \pi_i(\cdot \mid x,y_{\le t})}
    [Q_{\pi^*}(x, y_{\le t}, y_{t+1})]$
%
% $\pi_{\text{expert}}(\cdot \mid x,y_{\le t})=\pi_I(\cdot \mid x, y_{\le t})$ where $$I=\arg\max_i \EE_{y_{t+1}\sim \pi_i(\cdot \mid x,y_{\le t})}[Q^{\pi^*}(x,y_{\le t+1})].$$
We also make the following assumption to state that for any prefix $x,y_{\le t}$, there is one correct model that achieves approximate optimal value function.
%

\begin{assumption}[Global Coverage Assumption]\label{ass: difference}
    For any $x, y_{\le t}$, there exists an $i \in [n]$ such that 
    %
    \begin{align}
    \Big|\mathbb{E}_{y_{t+1}\sim \pi_{i}(\cdot \mid x,y_{\le t})}[Q^{\pi^*}(x,y_{\le t+1})]-V^*(x,y_{\le t})\Big| \le \Delta,\label{eq:assumption}
    \end{align}
    %
    where $\Delta$ represents the error between the optimal policy and the candidate model. 
    %
    This assumption states that the expert set is assumed to be sufficiently expressive so that one expert always achieves an approximately optimal value.
    %
    % \zz{If we claim this assumption, then why do we need the router to be generator at the same time? There is some discussion later, but I am thinking maybe we can add some additional words here as well:}
    %
    % \zz{
    % This assumption should be interpreted as a sanity bound that characterizes the best-case behavior of purely token-level routing under unrealistically strong coverage conditions.
    % %
    % }
    This assumption can be regarded as a sanity bound that characterizes the best-case performance of purely token-level routing under unrealistically strong coverage conditions.
    It assumes the existence of a near-optimal expert at \textit{each token}.
    %
    %
\end{assumption}
%


%
%
Following the Assumption~\ref{ass: difference} and Lemma~\ref{lemma: pdl},  we can get 
\begin{align}
\EE_{x\sim \rho}\left[V^{\pi^*}(x) - V^{\pi}(x)\right] 
\le \sum_{t=0}^{T-1} \Delta = T\Delta,\label{eq: pdl application}
\end{align}
%
% which means that when $\Delta \le 1/T$ is small, our training approach can successfully approximate the optimal response and generate the output with near-optimal reward. 
which means that when $\Delta \le O(1/T)$, an idealized token-level routing policy can achieve near-optimal expected return under Assumption~\ref{ass: difference}.
%
% In contrast, Collab does not try to choose to maximize the Q-function. Instead, the action selection is defined by 
% $$a_h  = \arg\max_{a_h}\mathbb{E}_{y_{t+1}\sim \pi_{a_h}(\cdot \mid x, y_{\le t})}[Q_h^{\pi_{a_h}}(x, y_{\le t+1})].$$
% This mismatch can lead to very bad performance. In fact, suppose $r(x,y) = $ suppose the optimal actions are $\pi^* = \pi_{a_1}$ for $t \le H/2$ and $\pi^* = \pi_{a_2}$ for $t \ge H/2+1$, the Collab fails to find the optimal policy. 
The \eqnref{eq: pdl application} shows that a well-trained purely token-level routing mechanism can possibly recover a near-optimal trajectory by selecting the appropriate expert at each step. We also discuss the difference between our approach and the prior token-level collaboration approach Collab~\citep{chakraborty2025collab} in Appendix~\ref{appendix: theoretical comparison}.

However, 
it is worth noting that Assumption~\ref{ass: difference} is relatively strong, since it requires a global coverage that must hold for \emph{all} prefixes, including those that may not appear in the supervised training data. 
%
Because the router is trained only on trajectories generated by the expert policy, satisfying this condition requires generalization beyond the observed data. 
%
A more natural assumption is to make the assumption only on the data generated by optimal policy $\pi^*$. 
%
In the next section, we show that this relaxed assumption is insufficient for generating an approximately optimal response, demonstrating the fundamental limitations of purely token-level collaboration.
%

\subsection{Limitations of Purely Token-Level Collaboration}
In the previous subsection, we showed that router training can recover the ideal action. 
%
However, Assumption~\ref{ass: difference} must hold for every possible prefix $x,y_{\le t}$. 
%
This assumption is rather restrictive, as the routing network is trained solely on the training dataset and may therefore suffer from distribution shift. 
%
A more reasonable requirement is to enforce \eqnref{eq:assumption} only for \textit{good} prefixes $x, y_{\le t}$. We consider two types of prefixes to be good prefixes. First, any prefix $x,y_{\le t} \sim \pi^*$ is considered as a good prefix,  which we call the \textit{single policy coverage} assumption. 
Moreover, any prefix that has the possibility to generate a good response is also considered as a good prefix, which we call the \textit{Generalization Coverage} assumption. Together, these two types of prefixes are intended to characterize the kinds
of text commonly encountered in the training data.
%
However, under this weaker assumption, we show that although there may exist a way to select a candidate model that yields a near-optimal response, such selection rule cannot be recovered solely from observations of the value function $Q^{\pi^*}$.
%

\begin{theorem}\label{theorem:path}
    Denote $\{n_1,n_2,\cdots, n_t\}$ as a path of length $t$, where $n_i \in [n], 1\le i\le t$. 
    %
    Assume that all $\pi^*$ and $\{\pi_i\}_{i \in [m]}$ are deterministic policy, the response length is fixed as $T$, and the transition function is also deterministic.  
    %
    Suppose the learner's observation space $\cO_t$ contains $$o_t
= \Bigl\{ x,\, y_{\le t},\, \{ Q^{\pi^*}(x, y_{\le k}) \}_{k=1}^t, \{Q^{\pi^*}(x,y_{\le t}, y)\}_{y \in \cY}\Bigr\}.$$ at the visited states $(x,y_{\le t})$ during decoding.  
    %
    % Then, if we want to achieve $\varepsilon-$optimal policy, at least for exponential paths $P_1,\cdots, P_N$,  we should assume  
    % \begin{align*}
    %     \mathbb{E}_{x,y_t \sim \pi_{P_n}}\Big|\mathbb{E}_{y_{t+1}\sim \pi_{a}(\cdot \mid x,y_{\le t})}[Q_t^{\pi^*}(x,y_{\le t+1})]-\mathbb{E}_{y_{t+1}\sim \pi^*(\cdot \mid x,y_{\le t})}[Q_t^{\pi^*}(x,y_{\le t+1})]\Big| \le \varepsilon.
    % \end{align*}
    %
    Suppose $\Delta>0$ is a error constant.
    Then, there is a MDP such that no token-level routing algorithm $\mathcal{A}:\cO \mapsto [n]$ can achieve $V^{\pi_{\cA}}\ge V^{\pi^*} - T/2 + 2$ for all possible rewards in this MDP, even if we have the following two good properties: 
    %
    \begin{enumerate}[leftmargin=2em]
        \item \textbf{Existence of a Near-Optimal Path.}  
        There exists a small $\varepsilon \le \Delta \in [0,1]$ and  at least one possible token-level routing strategy $P^*=\{n_1^*, n_2^*, \cdots, n_T^*\}$ such that
        \begin{align}
            V^{\pi^*} = V^{P^*} + \varepsilon. \label{assum: 1 optimal path}
        \end{align}
    
        \item \textbf{Single Policy Coverage.}  
        For the optimal policy $\pi^*$, the error constant $\Delta \in [0,1]$ such that the following approximation holds:
        \begin{align} &\mathbb{E}_{x,y_t\sim\pi^*}
        \Big|
        \arg\max_i \mathbb{E}_{y_{t+1}\sim\pi_{i}(\cdot\mid x,y_{\le t})}
            \big[Q^{\pi^*}(x,y_{\le t+1})\big]
        -
        \mathbb{E}_{y_{t+1}\sim\pi^*(\cdot\mid x,y_{\le t})}
            \big[Q^{\pi^*}(x,y_{\le t+1})\big]
        \Big|
        \le \Delta.\label{assum: 2 single policy}
        \end{align}
        \item \textbf{Generalization Coverage} For any prefix $x, y_{\le t}$, if there exists a full response $x, y_{\le T}$ with prefix $x, y_{\le t}$ and 
        $R(x,y_{\le T})\ge V^{\pi^*}-\Delta$, we have 

        \begin{align}&\Big|
        \arg\max_i \mathbb{E}_{y_{t+1}\sim\pi_{i}(\cdot\mid x,y_{\le t})}
            \big[Q^{\pi^*}(x,y_{\le t+1})\big]
        -
        \mathbb{E}_{y_{t+1}\sim\pi^*(\cdot\mid x,y_{\le t})}
            \big[Q^{\pi^*}(x,y_{\le t+1})\big]
        \Big|
        \le \Delta.\label{assum: 3 generalization}\end{align}

    \end{enumerate}
\end{theorem}
%
The impossibility in Theorem~\ref{theorem:path} stems from an identifiability failure, where observing optimal values along trajectories generated by $\pi^*$ is insufficient to determine which expert actions actually realize those values.
%
This is actually closely related to known limitations in reinforcement learning and imitation learning, where value information or on-policy demonstrations alone do not uniquely identify optimal actions without additional realizability assumptions~\citep{kakade2002approximately, ross2011reduction, levine2021inductive}
%
In fact, due to this identifiability failure, this theorem implies that designing a reliable method for selecting the optimal model to produce the optimal response is inherently difficult. 
%
For example, Theorem~\ref{theorem:path} shows that using SFT to train a router that chooses the optimal model is not reliable, because this is essentially equivalent to use behavior cloning for learning the actions that maximize the optimal value function $Q^{\pi^*}$. 
%
The proof is provided in \appref{appendix:proof theorem path}.
%

\subsubsection{Benefits of Router Training}
From the previous theorem, we show that reliable performance cannot be guaranteed under single-policy coverage. 
%
The core difficulty is that even if a prefix that may lead to good response (theoretically, a state has a large value $Q^{\pi^*}$), this response may not be realizable by the available candidate models. 
%
For each token, the set of feasible actions is restricted by the fixed expert models. 
%
Consequently, whenever the optimal policy $\pi^*$ and the expert models are not perfectly aligned, the resulting approximation error becomes uncontrollable.
%

To address this issue, we add the logits of the router as a complementary component (\eqnref{eq:combine}) to the final logits and train the final logits
 to align with the optimal policy. This removes the need to assume that any expert alone attains near-optimal Q-values; instead, we assume that the total variation distance between the final policy and the optimal policy is bounded.
%
In fact, since our training is to align $\pi_{i}'$ with the expert data where $\log \pi_i' = \log \pi_i  + \log \pi_{\text{router}}$, we can assume
%
\begin{align*}
    \mathbb{E}_{x\sim \rho,y_{\le t} \sim \pi^*}[\arg\min_{i}\text{TV}(\pi_i'(\cdot \mid x,y_{\le t}), \pi^*(\cdot \mid x,y_{\le t}))] \le \Delta.
\end{align*}
%
Then, if at each position $t$, the policy $\pi$ chooses the expert $i$ that $\pi_i'$ minimizes the TV distance to the  optimal policy, from PDL we can get
%
\begin{align*}
    V^{\pi^*}-V^\pi&= \sum_{t=0}^T \mathbb{E}_{y_t\sim \mathbb{P}_t^{\pi^*}(\cdot \mid x)}\Big[\mathbb{E}_{y_{t+1}\sim \pi^*(\cdot \mid x,y_{\le t})}Q_h^{\pi}(x,y_{\le t}, y_{t+1}) -\mathbb{E}_{y_{t+1}\sim \pi(\cdot \mid x,y_{\le t})}Q_h^{\pi}(x,y_{\le t}, y_{t+1})\Big]\\&\le TQ_{\max}\Delta.
\end{align*}
%
Hence, the discussion above shows that adding a router as a complementary part is a good way for overcoming the intrinsic difficulty for Theorem~\ref{theorem:path}. 
%
This result highlights an important conceptual shift. 
%
Instead of requiring that one of the fixed expert models be capable of achieving near-optimal performance on its own, we allow a router that serves both selection and complementation roles to compensate for the mismatch by contributing additional, adaptive logits. 
%
In this way, the combined policy effectively expands the expressivity of the action space, enabling it to approximate the optimal policy $\pi^*$ even when none of the individual candidate models is sufficient. 
%
This demonstrates that making the router a complementary component in the decoding process is not merely a heuristic enhancement, but a principled mechanism that circumvents the coverage assumption for all prefixes.
%

Furthermore, when the optimal policy and a candidate model are already reasonably well aligned, the router's complementary component need not be highly accurate; even a weakly informative router can suffice. 
%
In this case, the router is substantially easier to learn, as it only needs to correct the limited set of states where the candidate model deviates from $\pi^*$. 
%
On well-aligned states, the candidate models already provide strong responses. 
%
Consequently, combining a candidate model with a trainable router can outperform both fine-tuning a single model and pure routing. 
%
% \yh{I think in this part, you may want to state that training router with complementary role is not that hard but maybe that's not a thing that needs to emphasize?}\nuoya{I want to emphasize that why we do not only use the directly fine-tuned model. (In our theoretical analysis, we do not clarify the benefit of the existence of the candidate model.)}





% In practice, when the router assigns an incorrect expert at certain positions, the generated trajectory can deviate from the training data distribution, causing the router to fail to generalize effectively.  



% Hence, we also fine-tune the base model of the router to get an approximation $\pi_{router}\approx \pi^*.$ Now, instead of using the selected model $\pi$ solely for decoding, we use $\pi_{final}=\frac{1}{2}(\pi_{router} + \pi)$ by combine the router logits and the selected model logits.  This strategy can pull the trajectory back a bit to align with the optimal policy $\pi^*$.

% Now we make the relaxed assumption 
% \begin{assumption}
%     There exists a $\mathcal{R}: \mathcal{S} \mapsto  [M]$ such that for $\pi(\cdot \mid s_h) = \pi_{R(s_h)}(\cdot \mid s_h)$, we have 
%     $$\mathbb{E}_{s_t \sim \mathbb{P}_t^{\pi^*}(s_0), a_t \sim \pi(\cdot \mid s_h)}\left|Q_t^{\pi^*}(s_h,a_h) -V_t^{\pi^*}(s) \right| \le \Delta.$$
% \end{assumption}

% In fact, we now have 
% \begin{align*}V^{\pi^*}(s_0) - V^{\pi_{final}}(s_0) &= \sum_{h=0}^{H-1}\mathbb{E}_{s_h, a_h \sim \mathbb{P}_h^{\pi_{final}}(\cdot, \cdot \mid s_0)}\left[Q_h^{\pi^*}(s_h,a_h) -V_h^{\pi^*}(s) \right]\\
% &\le \sum_{h=1}^H \frac{\mathbb{P}_h^{\pi_{final}}(s_h)}{\mathbb{P}_h^{\pi^*}(s_h)}\mathbb{E}_{s_h \sim \mathbb{P}_h^{\pi^*}(s_0), a_h \sim \pi(\cdot \mid s_h)}\left|Q_h^{\pi^*}(s_h,a_h) -V_h^{\pi^*}(s) \right|\\
% &\le 2^H\sum_{h=1}^H H\Delta = 2H\Delta.\end{align*}







% \section{Multi-Objective Optimization}

% In this section, we discuss how to encourage collaboration among multiple agents in a multi-objective setting. Suppose we have several agents, each optimized for different objectives such as helpfulness and harmlessness. Our goal is to combine these agents with different weights, to generate responses that achieve a good Pareto frontier, effectively balancing the trade-offs between their respective objectives.

% Previous multi-objective algorithms, such as GenARM and MOD, typically fix a weight vector and generate the final response by combining the agents’ logits using these fixed weights. However, this approach lacks flexibility, as it assumes a constant trade-off across all tokens. In practice, the optimal weighting can vary at each decoding step, and adaptively adjusting the weights token-by-token may lead to better overall responses.

% Suppose we get $N$ agents $M_1, \cdots, M_N$ and $N$ normalized reward models $R_1,\cdots, R_N$. Previous algorithms always combine $N$ models as 
% $$\textbf{Logits} = \sum_{i=1}^N \alpha_i \textbf{Logits}(M_i).$$
% However, it is worth studying that whether it is beneficial to design adaptive weight. To be more specific, at the step $y_{\le t}, $ we can evaluate the objectives' score by the log-likelihood $$R_N(x,y_{\le t})=\sum_{i=1}^{t-1}\log \pi(y_{i}\mid x,y_{i-1}).$$ Then we can use these reward to decide the weight of linearly combining the models.
% For two models, we use 
% $$\alpha_t = \gamma \cdot \text{softmax}(-R_N) + (1-\gamma) \cdot [1,0]\  \text{or} \ [0,1]$$ for different $\gamma$ to represent different weights.
% If $\gamma = 1$, it means that  $\alpha_t = \gamma \cdot \text{softmax}(-R_N)$. In this case, for example, if $N=2$ and objectives are Helpful and Harmless, it means that we assign higher weights for helpful model if the previous response has lower likelihood for helpful model. This provides us an adaptive approach to allocate the weights for the model at the token-level. 

% \centerline{\includegraphics[scale=0.5]{frontier_with_two_lists.png}}

% The figure above shows the results for the multi-objective setting. The result shows that our approach can provide better result for max-min goal (maximize the minimum score).



% % One thing want to try: Use PPO to train the router directly. (Could be applicable for the unknown weight setting, and could be consistent for single-objective and multiple objective?)
